Improving Robustness of Learning-based Autonomous Steering Using Adversarial Images

For safety of autonomous driving, vehicles need to be able to drive under various lighting, weather, and visibility conditions in different environments. These external and environmental factors, along with internal factors associated with sensors, can pose significant challenges to perceptual data processing, hence affecting the decision-making and control of the vehicle. In this work, we address this critical issue by introducing a framework for analyzing robustness of the learning algorithm w.r.t varying quality in the image input for autonomous driving. Using the results of sensitivity analysis, we further propose an algorithm to improve the overall performance of the task of "learning to steer". The results show that our approach is able to enhance the learning outcomes up to 48%. A comparative study drawn between our approach and other related techniques, such as data augmentation and adversarial training, confirms the effectiveness of our algorithm as a way to improve the robustness and generalization of neural network training for autonomous driving.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\newcommand{\lyz}[1]{\textcolor[rgb]{0.505, 0, 0.921}{[Laura: {#1}]}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/old/3-overview.tex <==
\section{Experiment Setup}

\subsection{Datasets}
\weizi{1. Introduce the datasets you used in this work: CityScapes, GTA, Nvidia, Udacity. Show samples of the datasets. Explain why you choose them (features of each dataset). Explain why you choose two of them for AV using \emph{mediated perception} and the other two for AV using \emph{end-to-end}. (we probably will introduce these two pipelines in the intro, so here we can assume readers already know them).}
In our work, we use Nvidia paired with Udacity for end-to-end approach. We choose to use them because the content of CityScapes and GTA are similar (driving in the city), which helps to reduce the domain gap between real and virtual dataset, and they all have ground-truth for segmentation task. Similar for Nvidia and Udacity, we use them because of the content similarity and the same steering angle labels. See examples of those datasets in Fig.\ref{fig:dataset_example}.

\laura{\textbf{Data Sources.} We use the dataset used in \cite{NVIDIA-Data} as our real world data set. This data set contains approximately 63,000 images, or about 25 minutes of driving. In terms of location, the data was recorded on urban/suburban roads near Rancho Palos Verdes and San Pedro California. Our virtual dataset is collected by Zhenye Na from the Udacity Self-Driving Car Simulator, which includes about 31,000 images. This dataset includes a suburban driving track environment. The creation of both datasets were inspired by "End-to-End Learning for Self-Driving Cars" by Bojarski et al. \cite{DBLP:journals/corr/BojarskiTDFFGJM16}. For our experiment, we focus on the steering angle as our label. Comparisons in distributions for each dataset are be visualized in figure ~\ref{fig_driving_data_distribution}}.

\begin{figure}[h]
\begin{center}
   \includegraphics[width=1\linewidth]{figures/dataset_samples.jpg}
\end{center}
   \caption{Sample images of the datasets. The CityScapes and GTA samples have similar contents, and Nvidia and Udacity samples have similar contents.}
\label{fig:dataset_example}
\end{figure}


\subsection{Image Realism}
In our work, we take image realism as image style and image quality. Both of them are important factors.

\subsubsection{Image Style}
\weizi{1. Explain why you want to transfer image styles in general. why real to virtual and virtual to real. What are the use cases of these transfers?} 
We take image style as the rendering effect of the image, e.g., the style of a real photo is different from the style of a simulated image. In autonomous driving, it is expensive to collect real world dataset and label them, especially for special cases like accident data. Generating dataset from simulators will be much easier, since all the ground-truth is known in the virtual world. However, so far we are not able to render exact the same effect as the real world photo taken by a camera, which may lead a domain gap between the virtual dataset and real dataset. If we know how image style will influence the learning results, we may be able to use virtual dataset to strengthen the real dataset and get better results. 


\weizi{2. Introduce the algorithms you used in this work for style transfer, i.e., CycleGan and CR. What are they? What kind of operations they do? and Where are they used? Why you choose them in this work but not other image style algorithms (if there are any)? Show samples of transferred images. }

To go over the style gap between virtual dataset and real dataset, we use several style transfer algorithm. One of them is learning-based method CycleGan. CycleGan is a generative model which can exchange the image style of two sets of unpaired images by using a forward and backward supervision, which is one of the most famous style transfer learning methods. 

Another method we use is a traditional method color remapping. It can change the original color distribution to target distribution. Specifically, we use Histogram Warping\cite{rubner2000earth} to transfer 3 channels from the original distribution to the target distribution independently in HSV space. We don't do independent Histogram Warping in RGB space since remapping Red, Green and Blue channels independently will lead to a color bias, while in HSV space remapping Hue, Saturation and Value channels independently will have less color bias.



\subsubsection{Image Quality}
\weizi{1. Explain the operations you will execute on images: blur, noise, distortion. Why these operations? Why not other operations? (mention one or two common ones to show we know them and give a reason why they are excluded) Explain exactly how are you going to do this operations. For example, how to blur? by how much? etc. Show samples. }
In our experiments, we focus on blur, noise, and distortion regarding to the image quality, since they are very important and common in real world computer vision applications. There are other factors that may influence the image quality, e.g., the illumination in the environment. However, the effect of illumination change can not be modeled easily. Simply change the mean strength by a constant bias or a constant scale can not present the scene in stronger or weaker illumination in real world application.

For the blur factor, we use Gaussian blur to be the blur kernel, and choose 3 different standard deviations to be 3 different blur level, which is related to the size of original image. We choose the standard deviations by first choosing the worst case that we think a camera in real world application can be empirically, then interpolate 2 values between 0 and this borderline.

For the noise factor, we use Gaussian noise to be the noise model, se mean to 0 and choose 3 different standard deviations to be 3 different noise level. Similarly, we choose the standard deviations by first choosing the worst case that we think a camera in real world application can be empirically, then interpolate 2 values between 0 and this borderline.

For the distortion factor, we use positive radial distortion[] (or Barrel distortion) to be the distortion model, since it's the most common distortion in real world camera, especially for large FOV fish-eye cameras. Same rule here, we choose the standard deviations by first choosing the worst case that we think a camera in real world application can be empirically, then interpolate 2 values between 0 and this borderline. Notice to use the radial distortion, the camera intrinsic matrix is required. But here since our target is to distort the original image, so the intrinsic matrix doesn't need to be the ture value, we can set the value we want.

All the specific values will be introduced in the experiment setup, for both the mediated perception approach and the end-to-end approach.

\subsection{Tasks, models, and metrics chosen}
Since the mediated perception approach and the end-to-end approach are different, we need to specify different tasks and models.

For the mediated perception approach, we choose segmentation task as the mediated perception results. The most suitable task should be the 3D perception task, but we don't choose this task for two reasons. One is currently there is no public virtual dataset which has 3D perception labels. And for existing simulators like Deepdrive, it's hard to get access to all the 3D objects in the scene. Another reason is, 3D perception task is related with camera calibration parameters. We need to do cross experiments between real and virtual dataset, they have different camera calibration parameters but few virtual datasets contains camera calibration parameters. For segmentation task, we have ground-truth for both real and virtual dataset, and the camera calibration parameters are no longer needed, and the segmentation result is also one kind of mediated perception result, and contains more useful information than other tasks like object identification or classification. Therefore we choose segmentation task here. We choose HOS (HRNetV2 + OCR + SegFix) as the model for Pixel-Level Segmentation Task since it's the best model so far on the CityScapes benchmark, and choose Mask-RCNN as the model for Instance-Level Segmentation Task since it's widely used but not the best. Generally we want to see the results of both state-of-the-art and normal models, since in practice there may not be a benchmark for a specific task and we need to know a general conclusion. We use mIoU (mean Intersection over Union) for HOS since its output is in pixel-level, and use mAP (mean Average Precision) for Mask-RCNN since it's output is in instance-level. mIoU and mAP are all standard metrics for these specific tasks.

Similarly, for the end-to-end approach, we choose the regression task because of the property of dataset and the task itself. The input is image, and the output is steering angle (in degree). We use Nvidia model[] to do these experiments. Different from the metric used in the Nvidia paper[], we use MA (Mean Accuracy) and MSE (Mean Square Error) to evaluate the regression task, because the metric Nvidia paper used needs a simulator or a real autonomous driving car to do online test. Specifically, the Mean Accuracy is defined by the following equations.
$$
acc_{\tau}=\frac{count(|v_{pred} - v_{gt}|<\tau)}{n}
$$
Where $v_{pred}$ means the predicted value, $v_{gt}$ means the ground-truth, and $n$ means the total number of test case. 
Then
$$
MA = average_{\tau \in T}(acc_{\tau})
$$
Here we set $T=\{0.1, 0.2, 0.5, 1, 2, 5\}$ (in degree). We use MA metric here because it can represent an overall performance of the regression task with different tolerance, similar with mAP.

==> sections/old/4-experiment.tex <==
\section{Experiments}
In reality, it is hard to get large amount of labeled driving data under different situations, e.g., accident data, which we can get through simulator. However, the main problem of the synthetic data is the domain gap with the real world data. Here we focus on the image only. If we can transfer the synthetic image to a real world photo to reduce the domain gap, we can train a more accurate model with the help of it.

\subsection{Image Style Transfer}
Image style transfer is aiming to transfer the image style from one to another, e.g., from a photo-like image to a canvas. It becomes popular since the development of GAN[]. Recently CycleGan[] achieved an impressive performance in image style transfer. Here we use the CycleGan as the learning-based image style transfer method. In addition, we use color remapping as the classical method, which remaps the color of the source image to make the color distribution of the source image set to be similar with the target image set.


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\linewidth]{figures/segmentation_image_style.jpg}
\end{center}   
\caption{We show sample images from the datasets R (Real photos in Cityscapes dataset), \rvgan{} (Real photos in synthetic style generated by GAN), \rvcr (Real photos in synthetic style generated by color remapping) in the first row from left to right, and S (Synthetic images in GTA dataset), \vrgan (Synthetic images in real style generated by GAN), \vrcr (Synthetic images in real style generated by color remapping) in the second row from left to right.}
\label{fig_segmentation_image_style}
\end{figure}

\weizi{Explain why you include your datasets in the experiments, especially why you need GAN and CR transferred images, from real to virtual and vice versa.}  

notation: 

R: Real photos (Cityscapes dataset) %(cityscapes_ori)

V: Virtual images (GTA dataset) %(gta_ori)

GAN$_{R \rightarrow V}$: Real photos in synthetic style (GAN) %(cityscapes_fake_GAN)

\vrgan: Synthetic images in real style (GAN) %(gta_fake_GAN)

\rvcr: Real photos in synthetic style (Color Remapping) %(cityscapes_fake_color)

\vrcr: Synthetic images in real style (Color Remapping) %(gta_fake_color)

label(R)=label(\rvgan{})=label(\rvcr)

label(S)=label(\vrgan)=label(\vrcr)

label(R)!=label(S)

\weizi{Choose either table or figure to better illustrate your point. }
\begin{table}[ht] %(h = here, t = top)
    \caption{mAP comparison of MASK-RCNN on segmentation tasks (unit)}
    \label{tb_style_maskrcnn_unit}
    \centering
    \begin{tabular}{c|ccccccc}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}  \\  
        \cmidrule(l){2-7}     
        \multicolumn{1}{c}{Train} & R & V & \rvgan{} & \vrgan & \rvcr & \vrcr \\
        \midrule
            R & 25.68\% & 12.47\% & 25.08\% & 6.93\% & 19.02\% & 4.20\% \\
            V & 20.57\% & 26.91\% & 20.52\% & 24.21\% & 14.21\% & 23.37\% \\
            \rvgan{} & 26.18\% & 13.74\% & 27.83\% & 4.98\% & 19.24\% & 3.05\% \\
            \vrgan & 16.50\% & 18.60\% & 15.66\% & 25.00\% & 5.54\% & 25.24\% \\
            \rvcr & 21.03\% & 4.67\% & 23.67\% & 1.18\% & 29.44\% & 0.41\% \\
            \vrcr & 11.77\% & 3.51\% & 5.84\% & 18.28\% & 0\% & 21.77\% \\
        \bottomrule
    \end{tabular}
\end{table}

\textcolor{red}{Notation:(A, B) represent the results of training on A and testing on B.}

\textcolor{red}{Brief summary of Table.\ref{tb:style_maskrcnn_unit}:
\begin{itemize}
    \item There is domain gap between R and V. See (R, R), (R, V), (V, R), (V, V).
    \item Control the content of the image, use a different image style when testing (compare with training image style), the results may be nearly the same or decrease. See (R, R), (R, \rvgan{}), (\rvgan{}, R) as the similar case, and (R, R), (R, \rvcr), (\rvcr, R) as the decrease case.
    \item Transform the style of training virtual image to real style is not going to improve the test performance on the real data. See (V, R), (VR\_GAN, R), (VR\_CR). But in contrary, Transform the style of training real image to virtual style with Cycle-GAN can slightly improve the test performance on the virtual data. See (R, V), (RV\_GAN, V), (RV\_CR, V)
\end{itemize}
}


\begin{table}[ht] %(h = here, t = top)
  \caption{mIoU comparison of OpenSeg on segmentation tasks (unit)}
  \label{tab_style_openseg_unit}
    \centering
    \begin{tabular}{c|ccccccc}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}  \\  
        \cmidrule(l){2-7}     
        \multicolumn{1}{c}{Train} & R & S & \rvgan{} & \vrgan & \rvcr & \vrcr \\
        \midrule
            R & 72.15\% & 23.46\% & 29.42\% & 32.17\% & 30.79\% & 29.73\% \\
            S & 16.27\% & 42.56\% & 38.20\% & 7.19\% & 35.79\% & 13.09\% \\
            \rvgan{} & 29.59\% & xxx\% & 59.89\% & xxx\% & 41.42\% & xxx\% \\
            \vrgan & xxx\% & xxx\% & xxx\% & xxx\% & xxx\% & xxx\% \\
            \rvcr & 51.63\% & 33.80\% & 62.96\% & xxx\% & 74.93\% & 15.74\% \\
            \vrcr & 8.61\% & 14.15\% & 12.73\% & 9.58\% & 8.15\% & 12.46\% \\
        \bottomrule
    \end{tabular}
\end{table}

x

x

\textcolor{red}{Brief summary of Table.\ref{tb:style_maskrcnn_unit} and Table.\ref{tab_style_openseg_unit}:
\begin{itemize}
    \item Given the same datasets, the impact of image style may be different for different algorithms. We are using exactly the same datasets in Mask-RCNN experiments and OpenSeg experiments. But in Table. \ref{tab_style_openseg_unit} we can find the (R, \rvgan{}) and (\rvgan{}, R) is no longer similar with (R, R), which is different from that in Table.\ref{tb:style_maskrcnn_unit}.
\end{itemize}
 It will be good if we can find a metric to evaluate the similarity of two image styles in a given algorithm, like f(R, \rvgan{}, Mask-RCNN), but it's not easy to quantify image style in a general way. Maybe we can estimate the f in a specific task by doing enough experiments, but it's hard to find a general f.
}

\begin{table}[ht]
  \caption{mAP comparison of MASK-RCNN on segmentation tasks (combination)}
  \label{tab_style_maskrcnn_comb}
  \centering
  \begin{tabular}{c|cc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Test}                   \\
    \cmidrule(r){2-3}
    \multicolumn{1}{c}{Train} & R & S \\
    \midrule
            S + R & 19.64\% & 26.15\% \\
            \vrgan + R & 23.77\% & 12.47\% \\
            \vrcr + R & 13.03\% & 11.79\% \\
            S + \vrcr + \vrgan + R & 21.15\% & 22.64\% \\
            S & 20.57\% & 26.91\% \\
            R & 25.68\% & 12.47\% \\
            S(pretrain) + R & 30.03\% & 15.50\% \\
            \vrgan(pretrain) + R & 26.79\% & 9.00\% \\
            \vrcr(pretrain) + R & 25.79\% & 8.63\% \\
            (S + \vrcr + \vrgan)(pretrain) + R & 25.23\% & 10.37\% \\
            S(pretrain) + 0.5R & 30.37\% & 13.28\% \\
            S(pretrain) + 0.25R & 30.23\% & 10.91\% \\
            S(pretrain) + 0.1R & 28.54\% & 15.66\% \\
            S(pretrain) + 0.03R & 27.14\% & 15.37\% \\
            S(pretrain) + 0.01R & 23.45\% & 11.09\% \\
            S(pretrain) + 0.003R & 15.95\% & 09.06\% \\
            S(pretrain) + 0.001R & 08.59\% & 03.13\% \\
            %0.5R & 21.45\% & 4.29\% \\
            %0.25R & 23.51\% & 7.65\% \\
            %0.1R & 25.34\% & 10.27\% \\
            %0.03R & 18.56\% & 4.51\% \\
            %0.01R & 22.32\% & 4.62\% \\
            %0.003R & 14.48\% & 1.22\% \\
            %0.001R & 9.65\% & 00.17\% \\
    \bottomrule
  \end{tabular}
\end{table}

\textcolor{red}{Brief summary of Table.\ref{tab_style_maskrcnn_comb}:
\begin{itemize}
    \item Simply combine the training set of synthetic dataset and real dataset may decrease the performance, because of the domain gap. See (R, R), (S+R, R), (\vrgan+R, R), (\vrcr+R, R), (S+\vrcr+\vrgan+R, R).
    \item Using pretrain is better than simply combining the training data together when there's a domain gap. See (S+R, R), (\vrgan+R, R), (\vrcr+R, R), (S+\vrcr+\vrgan+R, R), (S(pretrain)+R, R), (\vrgan(pretrain)+R, R), (\vrcr(pretrain)+R, R), ((S+\vrcr+\vrgan)(pretrain)+R, R).
    \item Pretrain on synthetic dataset then train on real dataset may improve the performance, and such improvement can be achieved by using less data. See (R, R), (S(pretrain)+R, R), (S(pretrain)+R, 0.5R), (S(pretrain)+R, 0.25R), (S(pretrain)+R, 0.1R), (S(pretrain)+R, 0.03R).
\end{itemize}
}

\begin{table}[ht]
  \caption{mAP comparison of MASK-RCNN on segmentation tasks in different image qualities (\%)}
  \label{tab_quality_maskrcnn_unit}
  \centering
  \begin{tabular}{c|cccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{10}{c}{Test}                   \\
    \cmidrule(r){2-11}
    \multicolumn{1}{c}{Train} & R & B1 & B2 & B3 & N1 & N2 & N3 & D1 & D2 & D3 \\
    \midrule
            R & 25.68 & 25.15 & 23.90 & 22.69 & 20.57 & 3.33 & 2.00 & 27.11 & 27.56 & 19.46 \\
            \bOne{} & 23.48 & 24.58 & 24.72 & 24.34 & - & - & - & - & - & - \\
            \bTwo{} & 19.47  & 20.90 & 22.00 & 21.05 & - & - & - & - & - & - \\
            \bThree{} & 19.84  & 21.48 & 23.05 & 24.29 & - & - & - & - & - & -  \\
            \nOne{} & 26.97  & - & - & - & 25.54 & 05.36 & 00.03 & - & - & -  \\
            \nTwo{} & 23.20  & - & - & - & 22.70 & 22.94 & 00.71 & - & - & -  \\
            \nThree{} & 12.49  & - & - & - & 15.01 & 20.96 & 23.75 & - & - & -  \\
            \dOne{} & 25.76  & - & - & - & - & - & - & 29.86 & 29.72 & 27.79  \\
            \dTwo{} & 14.97  & - & - & - & - & - & - & 16.44 & 25.10 & 25.70  \\
            \dThree{} & 12.80  & - & - & - & - & - & - & 13.57 & 14.97 & 29.73  \\
    \bottomrule
  \end{tabular}
\end{table}

\textcolor{red}{Brief summary of Table.~\ref{tab_quality_maskrcnn_unit}:
\begin{itemize}
    \item Testing on a more blurred or less blurred dataset will decrease the performance. See the 4x4 cross experiments on R, B1, B2, B3. Original image is 2048x1024. Using Gaussian Blur, kernel size: B1:15x15, B2:35x35, B3:75x75.
    \item Testing on a more noisy or less noisy dataset will decrease the performance, and testing on a more noisy dataset may decrease the performance more dramatically than testing on a less noisy dataset. See the 4x4 cross experiments on R, N1, N2, N3. Using Gaussian Noise, 0 mean, sigma: N1:20, N2:50, N3:100.
    \item Testing on a more distorted or less distorted dataset will decrease the performance, and testing on a less distorted dataset may decrease the performance more dramatically than testing on a more distorted dataset. See the 4x4 cross experiments on R, D1, D2, D3. Using OpenCV camera distortion model, (k1,k2): D1:(0.01, 0.01), D2:(0.1, 0.1), D3:(1, 1).
\end{itemize}
}


\begin{table}[ht]
  \caption{mIoU comparison of OpenSeg on segmentation tasks in different image qualities (\%)}
  \label{tab_quality_openseg_unit}
  \centering
  \begin{tabular}{c|cccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{10}{c}{Test}                   \\
    \cmidrule(r){2-11}
    \multicolumn{1}{c}{Train} & R & B1 & B2 & B3 & N1 & N2 & N3 & D1 & D2 & D3 \\
    \midrule
            R & 72.15 & 57.91 & 22.30 & 15.67 & 51.27 & 19.54 & 12.10 & xxxx & xxxx & xxxx \\
            \bOne{} & 57.45 & 56.81 & 25.32 & 20.43 & - & - & - & - & - & - \\
            \bTwo{} & 28.17 & 36.22 & 46.98 & 44.00 & - & - & - & - & - & - \\
            \bThree{} & 23.72 & 30.24 & 41.29 & 52.33 & - & - & - & - & - & -  \\
            \nOne{} & 49.26 & - & - & - & 56.95 & 50.70 & 22.45 & - & - & -  \\
            \nTwo{} & 39.69 & - & - & - & 47.41 & 55.34 & 35.85 & - & - & -  \\
            \nThree{} & 7.66 & - & - & - & 7.66 & 7.68 & 17.34 & - & - & -  \\
            \dOne{} & xxxx & - & - & - & - & - & - & xxxx & xxxx & xxxx  \\
            \dTwo{} & xxxx & - & - & - & - & - & - & xxxx & xxxx & xxxx  \\
            \dThree{} & xxxx & - & - & - & - & - & - & xxxx & xxxx & xxxx  \\
    \bottomrule
  \end{tabular}
\end{table}

\textcolor{red}{Brief summary of Table.\ref{tab_quality_maskrcnn_unit} and Table.\ref{tab_quality_openseg_unit}:
\begin{itemize}
    \item Testing on a different blur level or noise level or distortion level will decrease the performance in both tables.
    \item The impact level of these factors may be different in different algorithms, e.g., See row \nOne{} and row \nThree{} in both tables.
\end{itemize}
The factors here are easier to quantify than image style. It's possible to draw a figure to show how the results changes when we change the blur level, noise level or distortion level. But we may need more samples for each factor.
}

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/segmentation_image_quality}
\end{center}   
\caption{We show sample images from the datasets in different qualities. We regenerate the dataset by blurring, noising and distorting the dataset in 3 levels.}
\label{fig_segmentation_image_quality}
\end{figure}

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/driving_image_stype}
\end{center}   
\caption{We show sample images from the datasets R (Real photos in Nvidia dataset), \rvgan{} (Real photos in synthetic style generated by GAN), \rvcr (Real photos in synthetic style generated by color remapping) in the first row from left to right, and S (Synthetic images in Udacity dataset), \vrgan (Synthetic images in real style generated by GAN), \vrcr (Synthetic images in real style generated by color remapping) in the second row from left to right.}
\label{fig_driving_image_stype}
\end{figure}



should notice the blur one, now most of the true positive case is road and building (large area), so blur may not influence that much. but things may change if we need small object segmentation

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\linewidth]{figures/driving_image_quality.jpg}
\end{center}   
\caption{We show sample images from the datasets in different qualities. We regenerate the dataset by blurring, noising and distorting the dataset in 3 levels.}
\label{fig_driving_image_quality}
\end{figure}


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\linewidth]{figures/distribution.png}
\end{center}   
\caption{Steering angle distribution of driving data. \laura{"Udacity" is collected from the Udacity Self-Driving Car Simulator, "NVIDIA" is a real-world dataset made available bY NVIDIA Corporation, and "Custom" is data collected from an in-house driving simulator based in Unity game engine. We consider the differences in data distribution as an indicator of inherent differences between real-world and virtual data. While Udacity and NVIDIA data seems similar in distribution, our custom dataset has values that are much more spread out negative values. (Yu, should we include our custom data here? No right turns were made)}}
\textcolor{red}{No, at least not now. Because now we can not improve the performance on NVIDIA with Udacity, which has smaller domain gap. A larger domain gap dataset is harder to handle.}
\label{fig_driving_data_distribution}
\end{figure}

Driving task

input: image

output: steering angle (1 float, in degree)

Mean Accuracy: if abs(prediction - groundtruth) < threshold then count it as a true positive case. We can get accuracy for one certain threshold. We use threshold=[0.1, 0.2, 0.5, 1, 2, 5]

example:

accuracy (+-0.100): 0.61607

accuracy (+-0.200): 0.80000

accuracy (+-0.500): 0.92679

accuracy (+-1.000): 0.97143

accuracy (+-2.000): 0.98929

accuracy (+-5.000): 0.99821

mean accuracy: 0.88363

\begin{table}[ht]
  \caption{Mean Accuracy comparison of driving task (unit)}
  \label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test} \\
    \cmidrule(r){2-7}
    \multicolumn{1}{c}{Train} & \rBase{} & \vBase{} & \rvgan{} & \vrgan{} & \rvcr{} & \vrcr{} \\
    \midrule
            \rBase{} & 88.36\% & 41.42\% & 51.42\% & 52.43\% & 60.89\% & 40.87\% \\
            \vBase{} & 31.16\% & 53.72\% & 34.22\% & 43.43\% & 35.86\% & 45.29\% \\
            \rvgan{} & 48.83\% & 44.09\% & 80.08\% & 40.09\% & 48.18\% & 42.03\% \\
            \vrgan{} & 26.87\% & 33.76\% & 29.34\% & 50.02\% & 27.79\% & 30.59\% \\
            \rvcr{} & 70.17\% & 47.81\% & 53.18\% & 47.83\% & 85.50\% & 40.24\% \\
            \vrcr{} & 30.08\% & 33.76\% & 38.86\% & 50.02\% & 37.41\% & 30.59\% \\
    \bottomrule
  \end{tabular}
\end{table}


\textcolor{red}{Brief summary of Table.\ref{tab_style_driving_unit}:
\begin{itemize}
    \item There is a domain gap between real data and synthetic data. See (R, R), (R, S), (S, R), (S, S).
    \item Control the content of the image, use a different image style when testing (compare with training image style),  the results may decrease. See (R, R), (R,\rvgan{}), (\rvgan{}, R) or (R, R), (R, \rvcr), (\rvcr, R) as the decrease case.
\end{itemize}
Show the image style will not only influence the segmentation task, but also influence the driving task.
}


\begin{table}[ht]
  \caption{Mean Accuracy comparison of driving task (combination)}
  \label{tab_style_driving_comb}
  \centering
  \begin{tabular}{c|cc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Test} \\
    \cmidrule(r){2-3}
    \multicolumn{1}{c}{Train} & R & S \\
    \midrule
            S + R & 77.02\% & 61.63\% \\
            \vrgan + R & 75.44\% & 44.84\% \\
            \vrcr + R & 73.42\% & 51.81\% \\
            S + \vrcr + \vrgan + R & 70.14\% & 66.06\% \\
            S & 31.16\% & 53.72\% \\
            R & 88.36\% & 41.42\% \\
            S(pretrain) + R & 83.54\% & 46.28\% \\
            %S(pretrain) + 0.3R & 81.01\% & 46.85\% \\
            S(pretrain) + 0.1R & 82.95\% & 42.28\% \\
            %S(pretrain) + 0.03R & xxx\% & xxx\% \\
            S(pretrain) + 0.01R & 82.67\% & 44.29\% \\
            %S(pretrain) + 0.003R & xxx\% & xxx\% \\
            %S(pretrain) + 0.001R & 83.60\% & 47.23\% \\
            %0.3R & 87.70\% & 51.81\% \\
            0.1R & 88.45\% & 48.86\% \\
            %0.03R & 88.48\% & 43.56\% \\
            0.01R & 85.80\% & 53.44\% \\
            %0.003R & xxx\% & xxx\% \\
            %0.001R & 83.60\% & 47.23\% \\
            \vrgan(pretrain) + R & xxx\% & xxx\% \\
            \vrcr(pretrain) + R & xxx\% & xxx\% \\
            (S + \vrcr + \vrgan)(pretrain) + R & xxx\% & xxx\% \\
    \bottomrule
  \end{tabular}
\end{table}

x

x

x

x

x

x


x

x

x

x

x

x


x

x

x

x

x

x

x

x




\textcolor{red}{Brief summary of Table.\ref{tab_style_driving_comb}:
\begin{itemize}
    \item In driving task, simply combine synthetic training dataset with real dataset will also decrease the performance as in the segmentation task. See (R, R), (S+R, R), (\vrgan+R, R), (\vrcr+R, R), (S+\vrcr+\vrgan+R, R).
    \item Using pretrain does not improve the performance in driving task, because the synthetic driving dataset has larger domain gap (not only image style, but also the steering angle label generated by keyboard controlling). See (R, R), (S(pretrain)+R, R).
\end{itemize}
Show in different case, the pretrain may or may not improve the performance, depending on the pretrain data.
}

\begin{table}[ht]
  \caption{Mean Accuracy comparison of driving tasks in different image qualities (\%)}
  \label{tab_quality_driving_unit}
  \centering
  \begin{tabular}{c|cccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{10}{c}{Test}                   \\
    \cmidrule(r){2-11}
    \multicolumn{1}{c}{Train} & R & B1 & B2 & B3 & N1 & N2 & N3 & D1 & D2 & D3 \\
    \midrule
            R & 88.36 & 88.21 & 88.06 & 86.07 & 88.33 & 86.01 & 81.42 & 88.30 & 88.63 & 74.97 \\
            \bOne{} & 87.05 & 87.08 & 86.84 & 83.98 & - & - & - & - & - & - \\
            \bTwo{} & 89.10 & 89.16 & 89.34 & 86.42 & - & - & - & - & - & - \\
            \bThree{} & 86.16 & 86.16 & 85.74 & 87.70 & - & - & - & - & - & -  \\
            \nOne{} & 89.10 & - & - & - & 88.45 & 86.54 & 81.16 & - & - & -  \\
            \nTwo{} & 86.57 & - & - & - & 87.50 & 87.35 & 83.54 & - & - & -  \\
            \nThree{} & 66.63 & - & - & - & 66.72 & 66.19 & 66.22 & - & - & -  \\
            \dOne{} & 88.06  & - & - & - & - & - & - & 88.09 & 87.76 & 72.70  \\
            \dTwo{} & 88.60  & - & - & - & - & - & - & 88.95 & 88.92 & 75.14  \\
            \dThree{} & 75.56  & - & - & - & - & - & - & 75.62 & 76.75 & 89.01  \\
    \bottomrule
  \end{tabular}
\end{table}

\textcolor{red}{Brief summary of Table.\ref{tab_quality_driving_unit}:
\begin{itemize}
    \item The blur factor does not influence the driving task, which is different from the segmentation task.
    \item The noise and distortion factor influence the driving task performance less than that of segmentation task. Only level 3 noise and level 3 distortion influenced the results.
\end{itemize}
}


\textcolor{red}{Table.\ref{tab_style_driving_unit_mse}, Table.\ref{tab_style_driving_comb_mse}, and Table.\ref{tab_quality_driving_unit_mse} are just monitoring another metric (Mean Square Error), similar results with Table.\ref{tab_style_driving_unit}, Table.\ref{tab_style_driving_comb}, and Table.\ref{tab_quality_driving_unit}}


\begin{table}[h]
  \caption{Mean Square Error comparison of driving task (unit)}
  \label{tab_style_driving_unit_mse}
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}                   \\
    \cmidrule(r){2-7}
    \multicolumn{1}{c}{Train} & R & S & \rvgan{} & \vrgan & \rvcr & \vrcr \\
    \midrule
            R & 0.20 & 17.21 & 3.23 & 16.46 & 2.42 & 16.24 \\
            S & 23.33 & 13.66 & 22.49 & 21.19 & 16.05 & 19.01 \\
            \rvgan{} & 5.37 & 14.96 & 0.45 & 18.47 & 5.05 & 15.08 \\
            \vrgan & 19.97 & 19.85 & 15.74 & 9.80 & 16.76 & 22.97 \\
            \rvcr & 1.12 & 16.87 & 2.75 & 16.07 & 0.25 & 18.37 \\
            \vrcr & 25.00 & 19.85 & 12.91 & 9.80 & 12.49 & 22.97 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[ht]
  \caption{Mean Square Error comparison of driving task (combination)}
  \label{tab_style_driving_comb_mse}
  \centering
  \begin{tabular}{c|cc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Test}                   \\
    \cmidrule(r){2-3}
    \multicolumn{1}{c}{Train} & R & S \\
    \midrule
            S + R & 0.79 & 9.88 \\
            \vrgan + R & 1.34 & 16.04 \\
            \vrcr + R & 0.70 & 11.02 \\
            S + \vrcr + \vrgan + R & 2.08 & 10.43 \\
            S & 23.33 & 13.66 \\
            R & 0.20 & 17.21 \\
            S(pretrain) + R & 0.35 & 17.05 \\
            S(pretrain) + 0.3R & 0.33 & 16.32 \\
            S(pretrain) + 0.1R & 0.31 & 17.87 \\
            S(pretrain) + 0.03R & xxx & xxx \\
            S(pretrain) + 0.01R & 0.29 & 16.84 \\
            S(pretrain) + 0.003R & xxx & xxx \\
            S(pretrain) + 0.001R & 0.35 & 16.81 \\
            0.3R & 0.15 & 15.81 \\
            0.1R & 0.16 & 15.95 \\
            0.03R & 0.14 & 14.62 \\
            %0.01R & 0.20 & 16.49 \\
            %0.003R & xxx & xxx \\
            %0.001R & 0.35 & 16.81 \\
            \vrgan(pretrain) + R & xxx & xxx \\
            \vrcr(pretrain) + R & xxx & xxx \\
            (S + \vrcr + \vrgan)(pretrain) + R & xxx & xxx \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[ht]
  \caption{Mean Square Error comparison of driving tasks in different image qualities (\%)}
  \label{tab_quality_driving_unit_mse}
  \centering
  \begin{tabular}{c|cccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{10}{c}{Test} \\
    \cmidrule(r){2-11}
    \multicolumn{1}{c}{Train} & R & B1 & B2 & B3 & N1 & N2 & N3 & D1 & D2 & D3 \\
    \midrule
            R & 0.20 & 0.20 & 0.20 & 0.22 & 0.21 & 0.23 & 0.31 & 0.20 & 0.19 & 0.61 \\
            \bOne{} & 0.17 & 0.17 & 0.17 & 0.21 & - & - & - & - & - & - \\
            \bTwo{} & 0.16 & 0.16 & 0.16 & 0.19 & - & - & - & - & - & - \\
            \bThree{} & 0.16 & 0.16 & 0.17 & 0.16 & - & - & - & - & - & -  \\
            \nOne{} & 0.15 & - & - & - & 0.15 & 0.16 & 0.27 & - & - & -  \\
            \nTwo{} & 0.19 & - & - & - & 0.18 & 0.18 & 0.26 & - & - & -  \\
            \nThree{} & 1.25 & - & - & - & 1.21 & 1.44 & 1.74 & - & - & -  \\
            \dOne{} & 0.14  & - & - & - & - & - & - & 0.14 & 0.14 & 0.60  \\
            \dTwo{} & 0.14  & - & - & - & - & - & - & 0.14 & 0.13 & 0.50  \\
            \dThree{} & 0.48  & - & - & - & - & - & - & 0.47 & 0.41 & 0.16  \\
    \bottomrule
  \end{tabular}
\end{table}

% \textcolor{red}{Brief summary of Table.\ref{tab_style_driving_unit_mse}, Table.\ref{tab_style_driving_comb_mse}, and Table.\ref{tab_quality_driving_unit_mse}:
% \begin{itemize}
%     \item Just monitor another metric of driving task. Basically the same trend with Table.\ref{tab_style_driving_unit}, Table.\ref{tab_style_driving_comb}, and Table.\ref{tab_quality_driving_unit}
% \end{itemize}
% }

==> sections/old/4-results.tex <==
\section{Experiment Results}
In this section, we detail our experiments. A basic guideline is, we first only change the key factor we want to investigate and fix other factors, to see the correlation between different value of the key factor. Then we do combination test to explore whether there's a way to improve the performance by making full use of the datasets.

We use (A,B) to denote the results of training on dataset A and test on dataset B. 


\subsection{Mediated Perception}
In this section, we first introduce the common setup for the experiments, then detail each experiment with descriptions and result analysis.

\subsection{Setup}

In the mediated perception approach, CityScapes and GTA as two base datasets and generate new datasets based on them. We introduce the datasets used in our experiments, along with their notation:
\begin{itemize}
    \item R: CityScapes (real);
    \item V: GTA (virtual);
    \item \rvgan{}: CityScapes, but transfer the style to GTA with CycleGan (real to virtual);
    \item \vrgan{}: GTA, but transfer the style to CityScapes with CycleGan (virtual to real);
    \item \rvcr{}: CityScapes, but transfer the style to GTA with color remapping (real to virtual);
    \item \vrcr{}: GTA, but transfer the style to CityScapes with color remapping (virtual to real);
    \item B1: Blur the CityScapes with (15, 15) Gaussian kernel (equivalent to $\sigma=2.6$), given the image size (2048, 1024);
    \item B2: Blur the CityScapes with (35, 35) Gaussian kernel (equivalent to $\sigma=5.6$), given the image size (2048, 1024);
    \item B3: Blur the CityScapes with (75, 75) Gaussian kernel (equivalent to $\sigma=11.6$), given the image size (2048, 1024);
    \item N1: Add Gaussian noise to the CityScapes with Gaussian distribution $N(\mu=0, \sigma=20)$;
    \item N2: Add Gaussian noise to the CityScapes with Gaussian distribution $N(\mu=0, \sigma=50)$;
    \item N3: Add Gaussian noise to the CityScapes with Gaussian distribution $N(\mu=0, \sigma=100)$;
    \item D1: Distort the CityScapes with radial distortion $(k_1=0.1, k_2=0.1)$, given the image size (2048, 1024), focal length $f=1000$ and the principle point (1024, 512);
    \item D2: Distort the CityScapes with radial distortion $(k_1=1, k_2=1)$, given the image size (2048, 1024), focal length $f=1000$ and the principle point (1024, 512);
    \item D3: Distort the CityScapes with radial distortion $(k_1=10, k_2=10)$, given the image size (2048, 1024), focal length $f=1000$ and the principle point (1024, 512);
\end{itemize}


\weizi{Put all your results associated with the conventional pipeline here.}

[Any data preprocessing is conducted?]
\laura{Some data preprocessing was applied in order to ensure that the labels in each dataset were aligned to the same definition. We define the steering angle as the degree value that the steering wheel turns \textbf{(check with Yu for update on this)}. The Udacity and NVIDIA datasets had differences in metrics during data collection. The Udacity dataset recorded the normalized values of car wheel angles, while the NVIDIA dataset recorded the degree value that the steering wheel turns. In order to account for this discrepancy, we scaled the Udacity data by its maximum wheel angle value along with the steering ratio used to record the NVIDIA dataset. The NVIDIA dataset was recorded on a 2014 Honda Civic, which has a 15.06 to 1 steering ratio. The steering ratio is defined as the ratio between the turning of the steering wheel and the car wheels. The comparison in adjusted labels can be visualized in figure ~\ref{fig_driving_data_distribution}.}

\subsubsection{Experiment 1}
\weizi{State your motivation. Explain your evaluation metric. Present your results using table(s) or figure(s). Discuss your findings.}
In this experiment, we explore the effect of image style to segmentation task with HOS model and Mask-RCNN model. we change the style of the two base datasets, then train and test on those datasets to see the correlation between them.
[We can put HOS at first if needed]

\begin{table}[ht] %(h = here, t = top)
    \caption{mAP correlation of MASK-RCNN on segmentation task}
    \label{tb:style_maskrcnn_unit}
    \centering
    \begin{tabular}{c|ccccccc}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}  \\  
        \cmidrule(l){2-7}     
        \multicolumn{1}{c}{Train} & R & V & \rvgan{} & \vrgan & \rvcr & \vrcr \\
        \midrule
            R & 25.68\% & 12.47\% & 25.08\% & 6.93\% & 19.02\% & 4.20\% \\
            V & 20.57\% & 26.91\% & 20.52\% & 24.21\% & 14.21\% & 23.37\% \\
            \rvgan{} & 26.18\% & 13.74\% & 27.83\% & 4.98\% & 19.24\% & 3.05\% \\
            \vrgan & 16.50\% & 18.60\% & 15.66\% & 25.00\% & 5.54\% & 25.24\% \\
            \rvcr & 21.03\% & 4.67\% & 23.67\% & 1.18\% & 29.44\% & 0.41\% \\
            \vrcr & 11.77\% & 3.51\% & 5.84\% & 18.28\% & 0\% & 21.77\% \\
        \bottomrule
    \end{tabular}
\end{table}

From Table.\ref{tb:style_maskrcnn_unit}, we can find:
\begin{itemize}
    \item There is domain gap between real and virtual dataset, which meets common sense. See (R, R), (R, V), (V, R), (V, V), Fig.\ref{}.
    \item Control the content of the image, use a different image style when testing (compare with training image style), the results may be nearly the same or decrease. See (R, R), (R, \rvgan{}), (\rvgan{}, R) as the similar case, and (R, R), (R, \rvcr), (\rvcr, R) as the decrease case.
    \item Transform the style of training virtual image to real style with the method used is not going to improve the test performance on the real data. See (V, R), (VR\_GAN, R), (VR\_CR, R). But in contrary, Transform the style of training real image to virtual style with CycleGan can slightly improve the test performance on the virtual data. See (R, V), (RV\_GAN, V), (RV\_CR, V).
\end{itemize}


\begin{table}[ht] %(h = here, t = top)
  \caption{mIoU correlation of HOS on segmentation task}
  \label{tb:style_openseg_unit}
    \centering
    \begin{tabular}{c|ccccccc}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}  \\  
        \cmidrule(l){2-7}     
        \multicolumn{1}{c}{Train} & R & S & \rvgan{} & \vrgan & \rvcr & \vrcr \\
        \midrule
            R & 72.15\% & 23.46\% & 29.42\% & 32.17\% & 30.79\% & 29.73\% \\
            S & 16.27\% & 42.56\% & 38.20\% & 7.19\% & 35.79\% & 13.09\% \\
            \rvgan{} & 29.59\% & xxx\% & 59.89\% & xxx\% & 41.42\% & xxx\% \\
            \vrgan & xxx\% & xxx\% & xxx\% & xxx\% & xxx\% & xxx\% \\
            \rvcr & 51.63\% & 33.80\% & 62.96\% & xxx\% & 74.93\% & 15.74\% \\
            \vrcr & 8.61\% & 14.15\% & 12.73\% & 9.58\% & 8.15\% & 12.46\% \\
        \bottomrule
    \end{tabular}
\end{table}


By comparing Table.\ref{tb:style_maskrcnn_unit} with Table.\ref{tb:style_openseg_unit}, we can find not all the rules for Mask-RCNN fit the rules for HOS, given they are using exactly same datasets. in Table. \ref{tb:style_openseg_unit} we can find the (R, \rvgan{}) and (\rvgan{}, R) is no longer similar with (R, R), which is different from that in Table.\ref{tb:style_maskrcnn_unit}.

Therefore, the valuable conclusions for the experiment 1 is:
\begin{itemize}
    \item It's a common sense that image style will influence the learning results. Here we also show that he impact of image style to different models can be dramatically different, given exactly the same datasets and similar tasks.
    \item Image style matters, but transform the image style from training dataset to testing dataset with current methods (learning methods like CycleGan or traditional methods like color remapping) is likely not helpful to improve the performance.
\end{itemize}


[It will be good if we can find a metric to evaluate the similarity of two image styles in a given algorithm, like f(R, \rvgan{}, Mask-RCNN), but it's not easy to quantify image style in a general way. Maybe we can estimate the f in a specific task by doing enough experiments, but it's hard to find a general f.]

\subsubsection{Experiment 2}
\weizi{State your motivation. Explain your evaluation metric. Present your results using table(s) or figure(s). Discuss your findings.}
In this experiment, we explore different ways to combine virtual dataset and real dataset to make the test results on real dataset better, regarding to the image style factor.

\begin{table}[ht]
  \caption{mAP comparison of MASK-RCNN on segmentation tasks (combination)}
  \label{tab_style_maskrcnn_comb}
  \centering
  \begin{tabular}{c|cc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Test}                   \\
    \cmidrule(r){2-3}
    \multicolumn{1}{c}{Train} & R & S \\
    \midrule
            S + R & 19.64\% & 26.15\% \\
            \vrgan + R & 23.77\% & 12.47\% \\
            \vrcr + R & 13.03\% & 11.79\% \\
            S + \vrcr + \vrgan + R & 21.15\% & 22.64\% \\
            S & 20.57\% & 26.91\% \\
            R & 25.68\% & 12.47\% \\
            S(pretrain) + R & 30.03\% & 15.50\% \\
            \vrgan(pretrain) + R & 26.79\% & 9.00\% \\
            \vrcr(pretrain) + R & 25.79\% & 8.63\% \\
            (S + \vrcr + \vrgan)(pretrain) + R & 25.23\% & 10.37\% \\
            S(pretrain) + 0.5R & 30.37\% & 13.28\% \\
            S(pretrain) + 0.25R & 30.23\% & 10.91\% \\
            S(pretrain) + 0.1R & 28.54\% & 15.66\% \\
            S(pretrain) + 0.03R & 27.14\% & 15.37\% \\
            S(pretrain) + 0.01R & 23.45\% & 11.09\% \\
            S(pretrain) + 0.003R & 15.95\% & 09.06\% \\
            S(pretrain) + 0.001R & 08.59\% & 03.13\% \\
            %0.5R & 21.45\% & 4.29\% \\
            %0.25R & 23.51\% & 7.65\% \\
            %0.1R & 25.34\% & 10.27\% \\
            %0.03R & 18.56\% & 4.51\% \\
            %0.01R & 22.32\% & 4.62\% \\
            %0.003R & 14.48\% & 1.22\% \\
            %0.001R & 9.65\% & 00.17\% \\
    \bottomrule
  \end{tabular}
\end{table}

From Table.\ref{tab_style_maskrcnn_comb}, we can find:
\begin{itemize}
    \item Simply combine the training set of synthetic dataset and real dataset may decrease the performance, because of the domain gap. See (R, R), (S+R, R), (\vrgan+R, R), (\vrcr+R, R), (S+\vrcr+\vrgan+R, R).
    \item Using pretrain is better than simply combining the training data together when there's a domain gap. See (S+R, R), (\vrgan+R, R), (\vrcr+R, R), (S+\vrcr+\vrgan+R, R), (S(pretrain)+R, R), (\vrgan(pretrain)+R, R), (\vrcr(pretrain)+R, R), ((S+\vrcr+\vrgan)(pretrain)+R, R).
    \item Using style transferred virtual data as pretraining data is not as good as using the oringinal virtual data. A possible reason is the style transfer algorithm will add other unknown noise. See (S(pretrain)+R, R), (\vrgan(pretrain)+R, R), (\vrcr(pretrain)+R, R), ((S+\vrcr+\vrgan)(pretrain)+R, R).
    \item Pretrain on synthetic dataset then train on real dataset may improve the performance, and such improvement can be achieved by using less data. See (R, R), (S(pretrain)+R, R), (S(pretrain)+R, 0.5R), (S(pretrain)+R, 0.25R), (S(pretrain)+R, 0.1R), (S(pretrain)+R, 0.03R).
\end{itemize}


\subsubsection{Experiment 3}
In this experiment, we change the value of the image quality factor only and fix other variables, then train and test on different datasets with different value of the same factor. The correlation is shown in Table.\ref{tb:quality_maskrcnn_unit}.

\begin{table}[ht]
  \caption{mAP correlation of MASK-RCNN on segmentation task with different image qualities (\%)}
  \label{tb:quality_maskrcnn_unit}
  \centering
  \begin{tabular}{c|cccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{10}{c}{Test}                   \\
    \cmidrule(r){2-11}
    \multicolumn{1}{c}{Train} & R & B1 & B2 & B3 & N1 & N2 & N3 & D1 & D2 & D3 \\
    \midrule
            R & 25.68 & 25.15 & 23.90 & 22.69 & 20.57 & 3.33 & 2.00 & 27.11 & 27.56 & 19.46 \\
            \bOne{} & 23.48 & 24.58 & 24.72 & 24.34 & - & - & - & - & - & - \\
            \bTwo{} & 19.47  & 20.90 & 22.00 & 21.05 & - & - & - & - & - & - \\
            \bThree{} & 19.84  & 21.48 & 23.05 & 24.29 & - & - & - & - & - & -  \\
            \nOne{} & 26.97  & - & - & - & 25.54 & 5.36 & 0.03 & - & - & -  \\
            \nTwo{} & 23.20  & - & - & - & 22.70 & 22.94 & 0.71 & - & - & -  \\
            \nThree{} & 12.49  & - & - & - & 15.01 & 20.96 & 23.75 & - & - & -  \\
            \dOne{} & 25.76  & - & - & - & - & - & - & 29.86 & 29.72 & 27.79  \\
            \dTwo{} & 14.97  & - & - & - & - & - & - & 16.44 & 25.10 & 25.70  \\
            \dThree{} & 12.80  & - & - & - & - & - & - & 13.57 & 14.97 & 29.73  \\
    \bottomrule
  \end{tabular}
\end{table}

From Table.~\ref{tb:quality_maskrcnn_unit}, we can find:
\begin{itemize}
    \item Testing on a more blurred or less blurred dataset will decrease the performance. See the 4x4 cross experiments on R, B1, B2, B3.
    \item Testing on a more noisy or less noisy dataset will decrease the performance, and testing on a more noisy dataset may decrease the performance more dramatically than testing on a less noisy dataset. See the 4x4 cross experiments on R, N1, N2, N3.
    \item Testing on a more distorted or less distorted dataset will decrease the performance, and testing on a less distorted dataset may decrease the performance more dramatically than testing on a more distorted dataset. See the 4x4 cross experiments on R, D1, D2, D3.
\end{itemize}

\begin{table}[ht]
  \caption{mIoU correlation of HOS on segmentation task with different image qualities (\%)}
  \label{tb:quality_openseg_unit}
  \centering
  \begin{tabular}{c|cccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{10}{c}{Test}                   \\
    \cmidrule(r){2-11}
    \multicolumn{1}{c}{Train} & R & B1 & B2 & B3 & N1 & N2 & N3 & D1 & D2 & D3 \\
    \midrule
            R & 72.15 & 57.91 & 22.30 & 15.67 & 51.27 & 19.54 & 12.10 & xxxx & xxxx & xxxx \\
            \bOne{} & 57.45 & 56.81 & 25.32 & 20.43 & - & - & - & - & - & - \\
            \bTwo{} & 28.17 & 36.22 & 46.98 & 44.00 & - & - & - & - & - & - \\
            \bThree{} & 23.72 & 30.24 & 41.29 & 52.33 & - & - & - & - & - & -  \\
            \nOne{} & 49.26 & - & - & - & 56.95 & 50.70 & 22.45 & - & - & -  \\
            \nTwo{} & 39.69 & - & - & - & 47.41 & 55.34 & 35.85 & - & - & -  \\
            \nThree{} & 7.66 & - & - & - & 7.66 & 7.68 & 17.34 & - & - & -  \\
            \dOne{} & xxxx & - & - & - & - & - & - & xxxx & xxxx & xxxx  \\
            \dTwo{} & xxxx & - & - & - & - & - & - & xxxx & xxxx & xxxx  \\
            \dThree{} & xxxx & - & - & - & - & - & - & xxxx & xxxx & xxxx  \\
    \bottomrule
  \end{tabular}
\end{table}

The valuable conclusions we can get from Table.\ref{tb:quality_maskrcnn_unit} and Table.\ref{tb:quality_openseg_unit}:
\begin{itemize}
    \item The impact level of these factors may be different in different algorithms, given exactly the same datasets and similar tasks, as shown in Fig.\ref{fig:correlation_comparison_noise}.
\end{itemize}

\begin{figure}[h]
\begin{center}
   \includegraphics[width=0.45\linewidth]{figures/maskrcnn_noise.jpg}
   \includegraphics[width=0.45\linewidth]{figures/hos_noise.jpg}
   \end{center}
   \caption{Correlation comparison between Mask-RCNN and mAP w.r.t. Noise. The shape of them is different, e.g., for Mask-RCNN, The main diagonal decreases slightly, while for the HOS, the main diagonal decreases dramatically. Also, Mask-RCNN perform bad on test N3 column when it's not trained on N3, while HOS perform bad when training on N3.}
\label{fig:correlation_comparison_noise}
\end{figure}

[The factors here are easier to quantify than image style. It's possible to draw a figure to show how the results changes when we change the blur level, noise level or distortion level. But we may need more samples for each factor.
Also, we can do combination test for image quality if we got time. The goal could be to train a model that have better performance on the levels of the same factor.]


\weizi{Summarize your findings from all experiments associated with the mediated perception pipeline.}


\subsection{End-to-end}
\weizi{Follow the same structure as the above. }


\weizi{Summarize your findings from all experiments (both systems). Make suggestions on how people in the community can use your findings and insights. }


==> sections/old/extra.tex <==
%While both datasets are similar in visual contents, the meanings of the labels differ. In the Nvidia dataset, the label is the steering angle, while in the Udacity dataset the label is the turning angle of the front wheels. We convert the labels in the Udacity dataset into steering angles by scaling them up by $15.06$, which is the steering-to-turning ratio of the 2014 Honda Civic~\cite{nvidia_steering_ratio}, the vehicle used to collect the Nvidia dataset. The maximum steering angle is 338 degrees. Sample images of the two datasets can be found in Fig.~\ref{fig:driving_image_style}(a) and Fig.~\ref{fig:driving_image_style}(b), respectively.  

% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\textwidth]{figures/samples.jpg}
% \end{center}   
% \caption{Sample images of various datasets. (a) the Nvidia dataset~\cite{NVIDIA-Data} (real dataset, denoted by \rBase{}). (b) the Udacity dataset~\cite{Udacity} (virtual dataset, denoted by \vBase{}). (c) style-transferred images from virtual to real using CycleGAN~\cite{Zhu2017} (denoted by \vrgan{}). (d) style-transferred images from virtual to real using MUNIT~\cite{huang2018multimodal} (denoted by \vrmunit{}). We plan to release all datasets for comparative experiments.}
% \label{fig:driving_image_style}
% \end{figure}


% , with a maximum turn angle of $\pm25$ degrees, but normalized to [-1,1]. In order to convert the labels of the Udacity dataset into steering angles, we first scale the original Udacity labels up by a factor of 25 and then

% We define the labels for these experiments to be the steering angle, i.e., the angle of the steering wheel turns. In order to account for these differences, we scaled the labels in the original Udacity dataset up by a factor of 25 (from normalized turning angle to true turning angle of the wheels), and then scaled by the steering ratio of the NVIDIA dataset $15.06$. This is because the vehicle used to record the dataset is a 2014 Honda Civic, which has a $15.06:1$ steering ratio~\cite{nvidia_steering_ratio}, with the ratio defined as degrees the steering wheel turns to the degrees the front wheels turn. In this way, we align all this labels to the same meaning, i.e., steering angle.




% Our task is steering angle controlling task, which is a regression task. The input is an image, and the output is the steering angle (in degree). We choose Nvidia model[] to do these experiments, which is already tested on a real AV in the on-road test. Different from the metric used in the Nvidia paper[], we use \MA{} (Mean Accuracy) to evaluate the regression task. We didn't use the metric in Nvidia paper because it needs a simulator or a real autonomous driving car to do online test. We use \MA{} metric here because it can represent an overall performance of the regression task with different tolerance, similar with mAP, while other metrics like MSE (Mean Square Error) do not have this property. Specifically, the Mean Accuracy is defined by the following equations.
% $$
% acc_{\tau}=\frac{count(|v_{pred} - v_{gt}|<\tau)}{n}
% $$
% Where $v_{pred}$ means the predicted value, $v_{gt}$ means the ground-truth, and $n$ means the total number of test cases. 
% Then
% $$
% \MA{} = average_{\tau \in T}(acc_{\tau})
% $$
% Here we set $T=\{0.1, 0.2, 0.5, 1, 2, 5\}$ (in degree). 


%\subsection{Image Quality}
% There are other factors that may influence the image quality, e.g., the illumination in the environment. However, the effect of illumination change can not be modeled easily. Simply change the mean strength by a constant bias or a constant scale can not present the scene in stronger or weaker illumination in real world application.

% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\linewidth]{figures/YUV.jpg}
% \end{center}   
% \caption{Sample images of channel level modification in YUV space. There 2 levels in the darker direction and 2 levels in the lighter direction.}
% \label{fig:driving_image_YUV}
% \vspace*{-1.2em}
% \end{figure}

% Notice that to use the radial distortion, the camera intrinsic matrix is required. But here since our target is to distort the original image, so the intrinsic matrix doesn't need to be the ture value, we can set the value we want.


%\subsection{Image Style}
% \weizi{1. Explain why you want to transfer image styles in general. why real to virtual and virtual to real. What are the use cases of these transfers?} 
% We take image style as the rendering effect of the image, e.g., the style of a real photo is different from the style of a simulated image. In autonomous driving, it is expensive to collect real world dataset and label them, especially for special cases like accident data. Generating dataset from simulators will be much easier, since all the ground-truth is known in the virtual world. However, so far we are not able to render exact the same effect as the real world photo taken by a camera, which may lead a domain gap between the virtual dataset and real dataset. If we know how image style will influence the learning results, we may be able to use virtual dataset to strengthen the real dataset and get better results. 


% \weizi{2. Introduce the algorithms you used in this work for style transfer, i.e., CycleGan and CR. What are they? What kind of operations they do? and Where are they used? Why you choose them in this work but not other image style algorithms (if there are any)? Show samples of transferred images. }

% \textbf{Image Style Transfer.} We use two style-transfer algorithms in this work. The first is CycleGAN~\cite{Zhu2017}, a generative model which can exchange the image style of two sets of unpaired images by using a forward and backward supervision. The second is MUNIT~\cite{huang2018multimodal}. This work assumes that the image representation can be decomposed into a domain-invariant content code and a domain-specific style code. An image then can be transferred from one domain to another by combining its invariant content code with a sampled style code from the target domain. We show sample images of the two types of style-transferred images in Fig.~\ref{fig:driving_image_style}(c) and Fig.~\ref{fig:driving_image_style}(d), respectively.




% \yu{here or related work?}
% There are other impressive GAN variations which can transfer image style, but may not be suitable for our case here. Pixel2Pixel HD~\cite{wang2018high} performs better than CycleGAN, but it needs paired images. CyCADA~\cite{hoffman2017cycada} is a follow-up work of CycleGAN which consists of pixel adaptation and feature adaptation, but the feature adaptation needs source task model, which is not a fair comparison here. VQVAE2~\cite{razavi2019generating} can generate images in target image set, but can not transfer the style of one image set to another, which is the requirements in our case. Therefore we finally choose CycleGAN and MUNIT as the style transfer algorithms in our experiments.

%Another method we use is a traditional method color remapping. It can change the original color distribution to target distribution. Specifically, we use Histogram Warping\cite{rubner2000earth} to transfer 3 channels from the original distribution to the target distribution independently in HSV space. We don't do independent Histogram Warping in RGB space since remapping Red, Green and Blue channels independently will lead to a color bias, while in HSV space remapping Hue, Saturation and Value channels independently will have less color bias.



% \textbf{Notation and Training Strategies.} In this work, we explore different ways to combine datasets in learning in order to test their potential to improve learning performance. We define the following notation for any two datasets $A$ and $B$. 

% \vspace*{-1em}
% \begin{itemize}
%     \item \train$(A+B)$: simply combine datasets $A$ and $B$ and use the combined dataset for training;
%     \item \pretrainTrain{$A$}{$B$}: use $A$ to pretrain a model,  then use $B$ to retrain the model; and
%     \item \pretrainPartialRetrain{$A$}{$B$}: use $A$ to pretrain a model, then use $B$ to retrain the model by only updating partial weights of the model. This training strategy is inspired by transfer learning~\cite{brownlee2018better}. Since we are using the model by Bojarski et al.~\cite{bojarski2016end}, we only update the weights in the fully connected layers during the retraining of the model using dataset $B$, while keeping the weights in the convolutional layers learned using dataset $A$. This operation is based on the assumption that the convolutional layers can extract domain-invariant, low-level features across different categories of images. 
% \end{itemize}

==> sections/old1/4.1-results1.tex <==
\vspace{-3pt}
\section{Experiment Results}
\vspace{-3pt}

In this section, we first demonstrate the experiment results associated with the quality reduction of real images in Sec.~\ref{sec:r}. Then, we present experiment results using virtual and real images in Sec.~\ref{sec:vr}. Last, we discuss the experiments results using all three styles of images, i.e., virtual, style-transferred, and real images in Sec.~\ref{sec:vtr}.

\vspace{-3pt}
\subsection{Quality Reduction of Real Images}
\label{sec:r}
\vspace{-3pt}
We first study how blur, noise, and distortion influence the performance of ``learning to steer''. The datasets used in this series of experiments are introduced by the following.  

\vspace*{-1em}
\begin{itemize}
    \item \rBase{}: real dataset (the Nvidia dataset~\cite{NVIDIA-Data});
    \item $B1, B2, B3, B4, B5$: Gaussian blur \rBase{} with standard deviation $\sigma=1.4$, $\sigma=2.9$, $\sigma=5.9$, $\sigma=10.4$, $\sigma=16.4$, which are equivalent to using kernel (7, 7), (17, 17), (37, 37), (67, 67), (107, 107), respectively;
    \item $N1, N2, N3, N4, N5$: add Gaussian noise to \rBase{} with $(\mu=0, \sigma=20)$, $(\mu=0, \sigma=50)$, $(\mu=0, \sigma=100)$, $(\mu=0, \sigma=150)$, $(\mu=0, \sigma=200)$, respectively;
    \item $D1, D2, D3, D4, D5$: distort \rBase{} with radial distortion $(k_1=1, k_2=1)$, $(k_1=10, k_2=10)$, $(k_1=50, k_2=50)$, $(k_1=200, k_2=200)$, $(k_1=500, k_2=500)$, respectively. $k_1$ and $k_2$ are radial distortion parameters; the focal length is $1000$; and the principle point is the center of the image.
\end{itemize}


The experiment results regarding \emph{blur} are summarized in Fig.~\ref{fig:driving_image_quality_blur}, with Fig.~\ref{fig:driving_image_quality_blur} LEFT showing the relative \MA{} values to \MADD{\rBase{}}{\rBasen{}}=88.36\% and Fig.~\ref{fig:driving_image_quality_blur} RIGHT showing the actual \MA{} values with \MADD{\rBase{}}{\rBasen{}}=88.36\% added. We find that when the training set and test set have lower (e.g., $\le B2$) or similar blur levels, the learning task is less influenced (i.e., the absolute value of relative \MA{} is close to 0). This phenomenon is pronounced when the training set and test set have the same blur level (see the diagonal values in Fig.~\ref{fig:driving_image_quality_blur} LEFT). This indicates that the learning algorithm can be trained and tested using very blurry images, while achieving the same performance as if the learning algorithm is trained and tested using non-blurry images. When the difference of the blur level between the training set and test set becomes higher, the learning task gets influenced more. However, the learning task is less sensitive to the blur effect in general as all values shown in Fig.~\ref{fig:driving_image_quality_blur} RIGHT are above 70\%.  



\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/MA_blur_combine.jpg}
\end{center}   
\caption{Experiment results regarding \emph{blur}. LEFT: relative \MA{} values to \MADD{\rBase{}}{\rBasen{}}=88.36\%. RIGHT: the landscape of actual \MA{} values (i.e., with \MADD{\rBase{}}{\rBasen{}}=88.36\% added). In general, the learning task is less sensitive to blurry images.}
\label{fig:driving_image_quality_blur}
\end{figure}


The experiment results regarding \emph{noise} are summarized in Fig.~\ref{fig:driving_image_quality_noise}. In contrast to blur, the learning task is less influenced only when the noise level is small (i.e., $\le N2$). Once the noise level becomes higher (i.e., >$N2$), the performance of the learning task drops substantially (e.g., relative \MA{} > 20\%). One interesting observation is that if the learning algorithm is trained using a dataset with low noise levels and tested using a dataset with high noise levels, the performance is better than that of the opposite operation. This indicates that the learning algorithm is more sensitive to the noise level of the training data, as opposed to the noise levels of the test data.



% For noise factor, there is not too much differences when adding the Gaussian noise to each pixel with standard deviation $\sigma<=50$,which is level <= 2 (<3\% in our experiments). But there is a dramatic decrease (nearly 20\%) when change the noise level from level 2 ($\sigma=50$) to level 3 ($\sigma=100$). An interesting observation is, the performance of training on smaller noise and testing on larger noise will be better than inverse, since numbers in top right triangular is larger than those in bottom left triangular, e.g., (\rBase{}, N5)=-15.21\%>(N5,\rBase{})=-34.53\%.
% With the increasing of noise, even training and testing on the same noise level, the performance will still decrease, see main diagnal [0, 0.09, -1.01, -22.14, -28.19, -34.02]. Train on low noise and test on high noise will be better than inverse.

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/MA_noise_combine.jpg}
\end{center}   
\caption{Experiment results regarding \emph{noise}. LEFT: relative \MA{} values to \MADD{\rBase{}}{\rBasen{}}=88.36\%. RIGHT: the landscape of actual \MA{} values (i.e., with \MADD{\rBase{}}{\rBasen{}}=88.36\% added). In general, the learning task is more sensitive to noisy images, compared to blurry images.}
\label{fig:driving_image_quality_noise}
\end{figure}



The experiment results regarding \emph{distortion} are summarized in Fig.~\ref{fig:driving_image_quality_distortion}. Similar to the blur effect, when the training set and test set have the same distortion levels, the learning task is less influenced (see the diagonal values in Fig.~\ref{fig:driving_image_quality_distortion} LEFT). However, when there is a gap between the distortion level of the training set and test set, the performance of the learning task responds dramatically. This indicates that among the three effects, the learning task is most sensitive to distortion. 

% For the distortion factor, when the distortion is small (level 1, $k_1=k_2=1$ in our case), the performance is influenced slightly (even slightly better in our case). For higher level, different distortion level of training and testing dataset, will lead to the performance loss decrease dramatically, while for the same level of training and testing dataset, it can still perform similar with the baseline. Different distortion level will influence the performance dramatically.

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/MA_distortion_combine.jpg}
\end{center}   
\caption{Experiment results regarding \emph{distortion}. LEFT: relative \MA{} values to \MADD{\rBase{}}{\rBasen{}}=88.36\%. RIGHT: the landscape of actual \MA{} values (i.e., with \MADD{\rBase{}}{\rBasen{}}=88.36\% added). This indicates that among the effects blur, noise, and distortion, the learning task is most sensitive to distortion.}
\label{fig:driving_image_quality_distortion}
\vspace*{-1em}
\end{figure}

% \begin{figure}[htb] 
%   \begin{minipage}[b]{0.65\textwidth} 
%       \centering
%       \begin{tabular}{c|cccccc}
%         \toprule
%         \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}                   \\
%         \cmidrule(r){2-7}
%         \multicolumn{1}{c}{Train} & \rBase{} & B1 & B2 & B3 & B4 & B5 \\
%         \midrule
%                 % \rBase{} & 88.36 & 88.21 & 88.06 & 86.07 & 81.16 & 73.33 \\
%                 % B1 & 87.05 & 87.08 & 86.84 & 83.98 & 78.78 & 70.92 \\
%                 % B2 & 89.10 & 89.16 & 89.34 & 86.42 & 83.89 & 73.98 \\
%                 % B3 & 86.16 & 86.16 & 85.74 & 87.70 & 84.07 & 77.02 \\
%                 % B4 & 82.58 & 82.76 & 83.21 & 85.03 & 87.64 & 81.66 \\
%                 % B5 & 76.45 & 76.33 & 76.57 & 78.57 & 82.58 & 88.51 \\
%                 \rBase{} & - & -0.15 & -0.3 & -2.29 & -7.2 & -15.03 \\
%                 B1 & -1.31 & -1.28 & -1.52 & -4.38 & -9.58 & -17.44 \\
%                 B2 & 0.74 & 0.8 & 0.98 & -1.94 & -4.47 & -14.38 \\
%                 B3 & -2.2 & -2.2 & -2.62 & -0.66 & -4.29 & -11.34 \\
%                 B4 & -5.78 & -5.6 & -5.15 & -3.33 & -0.72 & -6.7 \\
%                 B5 & -11.91 & -12.03 & -11.79 & -9.79 & -5.78 & 0.15 \\
%         \bottomrule
%       \end{tabular}
%       \caption{Experiment results regarding \emph{blur} measured using mean accuracy (MA) in percentages.}
%       \label{tab_quality_driving_unit}
%   \end{minipage}% 
%   \begin{minipage}[b]{0.38\textwidth} 
%     \begin{center}
%       \includegraphics[width=\textwidth]{figures/MA_blur.jpg}
%     \end{center}   
%     \caption{xxx}
%     \label{fig:driving_image_quality_all}
%   \end{minipage} 
% \end{figure}


% \begin{figure}[htb] 
%   \begin{minipage}[b]{0.65\textwidth} 
%   \centering
%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{c|cccccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}                   \\
%     \cmidrule(r){2-7}
%     \multicolumn{1}{c}{Train} & \rBase{} & N1 & N2 & N3 & N4 & N5 \\
%     \midrule
%             % \rBase{} & 88.36 & 88.33 & 86.01 & 81.42 & 76.39 & 73.15 \\
%             % N1 & 89.10 & 88.45 & 86.54 & 81.16 & 74.82 & 70.68 \\
%             % N2 & 86.57 & 87.50 & 87.35 & 83.54 & 78.30 & 73.33 \\
%             % N3 & 66.63 & 66.72 & 66.19 & 66.22 & 60.03 & 56.36 \\
%             % N4 & 58.24 & 59.01 & 59.52 & 61.69 & 60.17 & 55.00 \\
%             % N5 & 53.83 & 54.88 & 54.49 & 57.39 & 56.75 & 54.34 \\
%             \rBase{} & - & -0.03 & -2.35 & -6.94 & -11.97 & -15.21 \\
%             N1 & 0.74 & 0.09 & -1.82 & -7.2 & -13.54 & -17.68 \\
%             N2 & -1.79 & -0.86 & -1.01 & -4.82 & -10.06 & -15.03 \\
%             N3 & -21.73 & -21.64 & -22.17 & -22.14 & -28.33 & -32 \\
%             N4 & -30.12 & -29.35 & -28.84 & -26.67 & -28.19 & -33.36 \\
%             N5 & -34.53 & -33.48 & -33.87 & -30.97 & -31.61 & -34.02 \\
%     \bottomrule
%   \end{tabular}
%   }
%   %\caption{Mean Accuracy comparison w.r.t. noise (\%)}
%   %\label{tab_quality_driving_unit}
%   \end{minipage}% 
%   \begin{minipage}[b]{0.35\textwidth} 
%     \begin{center}
%       \includegraphics[width=\columnwidth]{figures/MA_noise.jpg}
%     \end{center}   
%     %\caption{Landscape of Mean Accuracy comparison w.r.t. noise (\%).}
%     %\label{fig:driving_image_quality_all}
%   \end{minipage} 
%     \caption{Landscape of Mean Accuracy comparison w.r.t. noise (\%).}
%     \label{fig:driving_image_noise}
% \end{figure}


% \begin{figure}[htb] 
%   \begin{minipage}[b]{0.65\textwidth} 
%   \centering
%   \begin{tabular}{c|cccccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}                   \\
%     \cmidrule(r){2-7}
%     \multicolumn{1}{c}{Train} & \rBase{} & D1 & D2 & D3 & D4 & D5 \\
%     \midrule
%             % \rBase{} & 88.36 & 88.63 & 74.97 & 57.67 & 48.83 & 49.16 \\
%             % D1 & 88.60 & 88.92 & 75.14 & 60.11 & 58.36 & 60.08 \\
%             % D2 & 75.56 & 76.75 & 89.01 & 61.33 & 50.03 & 41.01 \\
%             % D3 & 61.10 & 60.89 & 62.02 & 86.36 & 56.07 & 54.31 \\
%             % D4 & 54.49 & 54.58 & 54.31 & 53.24 & 86.51 & 55.08 \\
%             % D5 & 42.97 & 42.85 & 42.64 & 42.53 & 42.76 & 85.83 \\
%             \rBase{} & - & 0.27 & -13.39 & -30.69 & -39.53 & -39.2 \\
%             D1 & 0.24 & 0.56 & -13.22 & -28.25 & -30 & -28.28 \\
%             D2 & -12.8 & -11.61 & 0.65 & -27.03 & -38.33 & -47.35 \\
%             D3 & -27.26 & -27.47 & -26.34 & -2 & -32.29 & -34.05 \\
%             D4 & -33.87 & -33.78 & -34.05 & -35.12 & -1.85 & -33.28 \\
%             D5 & -45.39 & -45.51 & -45.72 & -45.83 & -45.6 & -2.53 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Mean Accuracy comparison of driving tasks w.r.t. distortion (\%)}
%   \label{tab_quality_driving_unit}
%   \end{minipage}% 
%   \begin{minipage}[b]{0.38\textwidth} 
%     \begin{center}
%       \includegraphics[width=\textwidth]{figures/MA_distortion.jpg}
%     \end{center}   
%     \caption{Landscape of Mean Accuracy comparison w.r.t. distortion (\%).}
%     \label{fig:driving_image_quality_all}
%   \end{minipage} 
% \end{figure}










==> sections/old1/4.2-results2.tex <==
\subsection{Channel level perturbation}
\label{sec:channel}
We then explore how channel level perturbations influence the performance of "learning to steer". We do experiments on RGB, HSV, and YUV space. Here we show the table for the RGB space experiments (see HSV, YUV space results in appendix).


\begin{table}[h]
  \caption{Mean Accuracy cross comparison, with modified value in R, G, B channels. The second letter 'S' means Smaller (darker Lv 1):v->v/2, and 'L' means Larger (lighter Lv 1):v->(v+255)/2.}
  %\label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|ccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{7}{c}{Test} \\
    \cmidrule(r){2-8}
    \multicolumn{1}{c}{Train} & $R$ & $R_{RS}$ & $R_{RL}$ & $R_{GS}$ & $R_{GL}$ & $R_{BS}$ & $R_{BL}$\\
    \midrule
            $R$ & 88.36\% & 57.91\% & 52.14\% & 53.54\% & 51.16\% & 54.25\% & 52.47\% \\
            $R_{RS}$ & 63.57\% & 88.21\% & 57.14\% & 50.56\% & 54.04\% & 44.73\% & 56.10\% \\
            $R_{RL}$ & 61.90\% & 55.62\% & 88.24\% & 43.48\% & 56.93\% & 50.56\% & 52.76\% \\
            $R_{GS}$ & 76.96\% & 57.08\% & 52.58\% & 88.86\% & 68.54\% & 55.17\% & 48.09\% \\
            $R_{GL}$ & 70.11\% & 51.75\% & 60.35\% & 52.70\% & 87.76\% & 49.82\% & 56.99\% \\
            $R_{BS}$ & 67.05\% & 55.23\% & 51.54\% & 47.97\% & 54.82\% & 87.08\% & 61.31\% \\
            $R_{BL}$ & 65.41\% & 55.06\% & 34.04\% & 38.00\% & 52.02\% & 53.72\% & 86.31\% \\
    \bottomrule
  \end{tabular}
\end{table}



% \begin{table}[h]
%   \caption{Mean Accuracy cross comparison, with modified value in H, S, V channels. The second letter 'S' means Smaller (darker Lv 1):v->v/2, and 'L' means Larger (lighter Lv 1):v->(v+255)/2.}
%   %\label{tab_style_driving_unit}
%   \centering
%   \begin{tabular}{c|ccccccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{7}{c}{Test} \\
%     \cmidrule(r){2-8}
%     \multicolumn{1}{c}{Train} & $R$ & $R_{HS}$ & $R_{HL}$ & $R_{SS}$ & $R_{SL}$ & $R_{VS}$ & $R_{VL}$\\
%     \midrule
%             $R$ & 88.36\% & 63.57\% & 51.48\% & 73.00\% & 61.36\% & 44.49\% & 49.25\% \\
%             $R_{HS}$ & 52.94\% & 86.84\% & 47.29\% & 53.89\% & 51.33\% & 41.93\% & 32.61\% \\
%             $R_{HL}$ & 48.36\% & 54.67\% & 86.33\% & 52.44\% & 53.92\% & 52.47\% & 37.50\% \\
%             $R_{SS}$ & 41.22\% & 51.19\% & 53.92\% & 87.73\% & 52.05\% & 52.23\% & 50.77\% \\
%             $R_{SL}$ & 47.85\% & 62.35\% & 46.48\% & 43.60\% & 86.10\% & 48.60\% & 44.46\% \\
%             $R_{VS}$ & 45.17\% & 54.52\% & 60.08\% & 62.08\% & 53.27\% & 86.01\% & 44.52\% \\
%             $R_{VL}$ & 46.31\% & 56.63\% & 44.61\% & 59.34\% & 49.76\% & 45.26\% & 86.48\% \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}[h]
%   \caption{Mean Accuracy cross comparison, with modified value in Y, U, V channels. The second letter 'S' means Smaller (darker Lv 1):v->v/2, and 'L' means Larger (lighter Lv 1):v->(v+255)/2.}
%   %\label{tab_style_driving_unit}
%   \centering
%   \begin{tabular}{c|ccccccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{7}{c}{Test} \\
%     \cmidrule(r){2-8}
%     \multicolumn{1}{c}{Train} & $R$ & $R_{YS}$ & $R_{YL}$ & $R_{US}$ & $R_{UL}$ & $R_{VS}$ & $R_{VL}$\\
%     \midrule
%             $R$ & 88.36\% & 46.90\% & 51.25\% & 49.58\% & 48.21\% & 54.16\% & 47.44\% \\
%             $R_{YS}$ & 64.40\% & 88.51\% & 49.61\% & 53.24\% & 43.86\% & 49.67\% & 50.06\% \\
%             $R_{YL}$ & 61.69\% & 49.04\% & 87.11\% & 50.62\% & 56.75\% & 54.31\% & 52.76\% \\
%             $R_{US}$ & 71.54\% & 42.05\% & 57.02\% & 86.31\% & 61.16\% & 60.62\% & 47.79\% \\
%             $R_{UL}$ & 71.45\% & 49.46\% & 56.28\% & 64.85\% & 86.75\% & 51.33\% & 39.46\% \\
%             $R_{VS}$ & 70.41\% & 37.56\% & 53.18\% & 48.42\% & 61.48\% & 88.15\% & 59.10\% \\
%             $R_{VL}$ & 71.63\% & 42.94\% & 52.73\% & 53.27\% & 47.94\% & 61.69\% & 86.96\% \\
%     \bottomrule
%   \end{tabular}
% \end{table}


==> sections/old1/5.1-results.tex <==
\section{Results}

\subsection{Original gap}
If we just train on the original dataset R, we can see performance decrease with the increasing of perturbation levels.

We first study how blur, noise, and distortion influence the performance of ``learning to steer''. The datasets used in this series of experiments are introduced by the following.  

% \vspace*{-1em}
\begin{itemize}
    \item \rBase{}: real dataset (the Nvidia dataset~\cite{NVIDIA-Data});
    \item $B1, B2, B3, B4, B5$: Gaussian blur \rBase{} with standard deviation $\sigma=1.4$, $\sigma=2.9$, $\sigma=5.9$, $\sigma=10.4$, $\sigma=16.4$, which are equivalent to using kernel (7, 7), (17, 17), (37, 37), (67, 67), (107, 107), respectively;
    \item $N1, N2, N3, N4, N5$: add Gaussian noise to \rBase{} with $(\mu=0, \sigma=20)$, $(\mu=0, \sigma=50)$, $(\mu=0, \sigma=100)$, $(\mu=0, \sigma=150)$, $(\mu=0, \sigma=200)$, respectively;
    \item $D1, D2, D3, D4, D5$: distort \rBase{} with radial distortion $(k_1=1, k_2=1)$, $(k_1=10, k_2=10)$, $(k_1=50, k_2=50)$, $(k_1=200, k_2=200)$, $(k_1=500, k_2=500)$, respectively. $k_1$ and $k_2$ are radial distortion parameters; the focal length is $1000$; and the principle point is the center of the image.
\end{itemize}

First pick the proper range for each factor. Channel level range (0,255). blur, noise and distortion ranges are chosen empirically, according to the bad performance camera in the real world.
Then interpolate the values to make any two of them are different enough from parameter value level, image visual level (determined by human empirically), image pixel level and feature level (FID metric), and can also show the trend of the accuracy curve.


\begin{table}[ht]
  \caption{Original performance on different levels of blur, noise, and distortion.}
  \label{tb:style_driving_comb}
  \centering
  \begin{tabular}{c|ccccc}
    \toprule
factor & Lv.1 & Lv.2 & Lv.3 & Lv.4 & Lv.5\\
    \midrule
        blur  & 88.21\% & 88.06\% & 86.07\% & 81.16\% & 73.33\% \\
        noise & 88.33\% & 86.01\% & 81.42\% & 76.39\% & 73.15\% \\
        distortion  & 88.63\% & 74.97\% & 57.67\% & 48.83\% & 49.16\% \\
        % & G-channel(RGB)  & 53.54\% & 51.16\% & - & - & - \\
        % & S-channel(HSV)  & 73.00\% & 61.36\% & - & - & - \\
        % & Y-channel(YUV)  & 46.90\% & 51.25\% & - & - & - \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[ht]
  \caption{Original performance on different levels of R, G, B, and H, S, V.}
  \label{tb:style_driving_comb}
  \centering
  \begin{tabular}{c|cccc}
    \toprule
 factor & darker Lv.2 & darker Lv.1 & lighter Lv.1 & lighter Lv.2\\
    \midrule
        R & 53.24\% & 57.91\% & 52.14\% & 45.14\% \\
        G & 44.16\% & 53.54\% & 51.16\% & 39.97\% \\
        B & 43.03\% & 54.25\% & 52.47\% & 42.58\% \\
        H & 51.28\% & 63.57\% & 51.48\% & 51.22\% \\
        S & 58.36\% & 73.00\% & 61.36\% & 53.15\% \\
        V & xxx\% & 44.49\% & 49.25\% & 39.43\% \\
    \bottomrule
  \end{tabular}
\end{table}


==> sections/old1/5.1-results1.tex <==

\begin{table}[ht]
      \centering
      \caption{\BN{} statistics results of the blur effect. The \ltwo{} norm of \BNDD{\rBase{}}{D} and \BNDD{$D$}{\rBasen{}} to the baseline \BNDD{$R$}{\rBasen{}}, using the corresponding mean and standard deviation values are reported. In both (a) and (b), the absolute \MA{} difference is also shown for comparison. Overall, we find the \ltwo{} norm values correlate positively with the \MA{} difference. In addition, changing the blur level of the training dataset has higher influence on \ltwo{} norm than changing the blur level of the test dataset. Given $\|$\BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2=40.08$, $\|$\BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2=92.04$, and \MADD{\rBase{}}{\rBasen{}} $=88.36\%$.}      
      
      \begin{tabular}{cl|cccccc}
        \toprule
         & & &  \multicolumn{3}{c}{ Dataset ($D$)} \\
         & & $B1$ & $B2$ & $B3$ & $B4$ & $B5$\\
        \midrule
        & $\|$\BNDDC{\rBase{}}{D}{mean}$\|_2$ & 40.77 & 40.69 & 40.31 & 39.77 & 39.51 \\
        & $\|$\BNDDC{\rBase{}}{D}{mean} $-$ \BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2$ & 0.10 & 0.99 & 3.65 & 3.45 & 7.87 \\
        & $\Delta$\BNDDC{\rBase{}}{}{mean} $/$ $\|$
        \BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2$ & 0.23\% & 2.44\% & 8.93\% & 8.45\% & 19.29\% \\
        \cmidrule(r){2-7}
        & $\|$\BNDDC{\rBase{}}{D}{std}$\|_2$ & 91.91 & 91.87 & 88.20 & 86.17 & 79.66 \\
    (a) & $\|$\BNDDC{\rBase{}}{D}{std} $-$ \BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2$ & 0.18 & 0.58 & 4.26 & 7.50 & 14.63 \\
        & $\Delta$\BNDDC{\rBase{}}{}{std} $/$ $\|$ \BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2$ & 0.19\% & 0.62\% & 4.63\% & 8.14\% & 15.88\% \\
        \cmidrule(r){2-7}
        & \MADD{\rBase{}}{D}  & 88.21\% & 88.06\% & 86.07\% & 81.16\% & 73.33\% \\
        & $|$\MADD{\rBase{}}{D} $-$ \MADD{\rBase{}}{\rBasen{}}$|$ & 0.15\% & 0.3\% & 2.29\% & 7.2\% & 15.03\% \\
        & $\Delta$\MADD{\rBase{}}{} $/$ \MADD{\rBase{}}{\rBasen{}} & 0.17\% & 0.34\% & 2.59\% & 8.15\% & 17.01\% \\
        \midrule
        %Element & (B1, R) & (B2, R) & (B3, R) & (B4, R) & (B5, R)\\
        %\midrule
        & $\|$\BNDDC{$D$}{D}{mean}$\|_2$ & 30.34 & 43.39 & 42.23 & 41.24 & 46.63 \\
        & $\|$\BNDDC{$D$}{\rBasen{}}{mean}$\|_2$ & 30.37 & 43.65 & 42.43 & 42.43 & 48.80 \\
        & $\|$\BNDDC{$D$}{D}{mean} $-$ \BNDDC{$D$}{\rBasen{}}{mean}$\|_2$ & 0.08 & 1.18 & 4.18 & 3.05 & 9.15 \\
        & $\Delta$\BNDDC{$D$}{}{mean} $/$ $\|$ \BNDDC{$D$}{D}{mean}$\|_2$  & 0.27\% & 2.73\% & 9.90\% & 7.40\% & 19.62\% \\
        \cmidrule(r){2-7}
        & $\|$\BNDDC{$D$}{D}{std}$\|_2$ & 71.46 & 100.61 & 96.70 & 100.87 & 107.85 \\
    (b) & $\|$\BNDDC{$D$}{\rBasen{}}{std}$\|_2$ & 71.58 & 100.49 & 100.54 & 105.38 & 121.52 \\
        & $\|$\BNDDC{$D$}{D}{std} $-$ \BNDDC{$D$}{\rBasen{}}{std}$\|_2$ & 0.16 & 0.50 & 4.09 & 5.61 & 16.02 \\
        & $\Delta$\BNDDC{$D$}{}{std} $/$ $\|$ \BNDDC{$D$}{D}{std}$\|_2$ & 0.22\% & 0.50\% & 4.23\% & 5.56\% & 14.85\% \\
        \cmidrule(r){2-7}
        & \MADD{$D$}{D} & 87.08\% & 89.34\% & 87.70\% & 87.64\% & 88.51\% \\
        & \MADD{$D$}{\rBasen{}} & 87.05\% & 89.10\% & 86.16\% & 82.58\% & 76.45\% \\
        & $|$\MADD{$D$}{D} $-$ \MADD{$D$}{\rBasen{}}$|$  & 0.03\% & 0.24\% & 1.54\% & 5.06\% & 12.06\% \\
        & $\Delta$\MADD{$D$}{} $/$ \MADD{$D$}{D} & 0.03\% & 0.26\% & 1.75\% & 5.77\% & 13.62\% \\
        \bottomrule
      \end{tabular}
      \label{tab:bn_blur}
\end{table}
   %   We calculate the L2 norm of the BN statistics difference between \BNMD{$train(R)$}{\rBasen{}} (baseline) and \BNDD{\rBase{}}{D} / \BNDD{$D$}{\rBasen{}}, where $D \in \{B1, B2, B3, B4, B5\}$, and show L2 norm of mean difference and std difference in second row and third row, respectively. In the forth row, we show the absolute Mean Accuracy (\MA{}) difference between \MAMD{$train(R)$}{\rBasen{}} (baseline) and \MADD{\rBase{}}{D} / \MADD{$D$}{\rBasen{}}, where $D \in \{B1, B2, B3, B4, B5\}$. We can find no matter we increase the blur level of test dataset (upper part) or training dataset (bottom part), the L2 norm of Mean diff and Std diff increase with the increasing of the \MA{} diff, showing that they are positive related. In addition, changing the blur level of the training dataset will have larger BN mean and std differences than changing the blur level of the test dataset.


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/BN_ratio_blur.jpg}
\end{center}   
\caption{Curve for blur. Showing the MA percentage difference is nearly positive related to the the BN statistics percentage difference, including mean and std.}
\label{fig:BN_ratio_blur}
\end{figure}



\begin{table}[ht]
      \centering
      \caption{\BN{} statistics results of the noise effect. The \ltwo{} norm of \MADD{\rBase{}}{D} and \MADD{$D$}{\rBasen{}} to the baseline \BNDD{$R$}{\rBasen{}}, using the corresponding mean and standard deviation values are reported. In both (a) and (b), the absolute \MA{} difference is also shown for comparison. We find that when increasing the noise level of test dataset (a), the \ltwo{} norm increases as the absolute \MA{} difference increases. However, when increasing the noise level of the training dataset (b), similar behavior is not found. In addition, changing the noise level of the training dataset will result in larger \ltwo{} norm than changing the test dataset.}
      \begin{tabular}{cl|cccccc}
        \toprule
        & & &  \multicolumn{3}{c}{ Dataset ($D$)} \\
        & & $N1$ & $N2$ & $N3$ & $N4$ & $N5$\\
        \midrule
        & $\|$\BNDDC{\rBase{}}{D}{mean}$\|_2$ & 39.89 & 37.25 & 31.18 & 26.06 & 22.66 \\
        & $\|$\BNDDC{\rBase{}}{D}{mean} $-$ \BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2$ & 1.65 & 4.86 & 10.57 & 15.85 & 19.74 \\
        & $\Delta$\BNDDC{\rBase{}}{}{mean} $/$ $\|$
        \BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2$ & 4.05\% & 11.91\% & 25.92\% & 38.84\% & 48.37\% \\
        \cmidrule(r){2-7}
        & $\|$\BNDDC{\rBase{}}{D}{std}$\|_2$ & 90.49 & 85.33 & 72.06 & 60.03 & 51.10 \\
    (a) & $\|$\BNDDC{\rBase{}}{D}{std} $-$ \BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2$ & 1.62 & 6.79 & 20.04 & 32.10 & 41.05 \\
        & $\Delta$\BNDDC{\rBase{}}{}{std} $/$ $\|$ \BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2$ & 1.76\% & 7.37\% & 21.77\% & 34.87\% & 44.60\% \\
        \cmidrule(r){2-7}
        & \MADD{\rBase{}}{D}  & 88.33\% & 86.01\% & 81.42\% & 76.39\% & 73.15\% \\
        & $|$\MADD{\rBase{}}{D} $-$ \MADD{\rBase{}}{\rBasen{}}$|$ & 0.03\% & 2.35\% & 6.94\% & 11.97\% & 15.21\% \\
        & $\Delta$\MADD{\rBase{}}{} $/$ \MADD{\rBase{}}{\rBasen{}} & 0.03\% & 2.65\% & 7.85\% & 13.54\% & 17.21\% \\
        \midrule
        %Element & (B1, R) & (B2, R) & (B3, R) & (B4, R) & (B5, R)\\
        %\midrule
        & $\|$\BNDDC{$D$}{D}{mean}$\|_2$ 
        & 41.56 & 35.01 & 1.61 & 1.39 & 0.66 \\
        & $\|$\BNDDC{$D$}{\rBasen{}}{mean}$\|_2$ 
        & 42.50 & 38.24 & 2.18 & 2.01 & 1.04 \\
        & $\|$\BNDDC{$D$}{D}{mean} $-$ \BNDDC{$D$}{\rBasen{}}{mean}$\|_2$ 
        & 1.48 & 4.24 & 0.69 & 0.80 & 0.53 \\
        & $\Delta$\BNDDC{$D$}{}{mean} $/$ $\|$ \BNDDC{$D$}{D}{mean}$\|_2$  
        & 3.56\% & 12.13\% & 43.02\% & 57.99\% & 80.43\% \\
        \cmidrule(r){2-7}
        & $\|$\BNDDC{$D$}{D}{std}$\|_2$ 
        & 84.71 & 82.68 & 4.86 & 2.95 & 1.89 \\
    (b) & $\|$\BNDDC{$D$}{\rBasen{}}{std}$\|_2$ 
        & 86.23 & 89.69 & 6.36 & 4.56 & 2.60 \\
        & $\|$\BNDDC{$D$}{D}{std} $-$ \BNDDC{$D$}{\rBasen{}}{std}$\|_2$ 
        & 1.59 & 7.11 & 1.54 & 1.71 & 0.98 \\
        & $\Delta$\BNDDC{$D$}{}{std} $/$ $\|$ \BNDDC{$D$}{D}{std}$\|_2$ 
        & 1.88\% & 8.60\% & 31.72\% & 58.03\% & 51.98\% \\
        \cmidrule(r){2-7}
        & \MADD{$D$}{D} 
        & 88.45\% & 87.35\% & 66.22\% & 60.17\% & 54.34\% \\
        & \MADD{$D$}{\rBasen{}} 
        & 89.1\% & 86.57\% & 66.63\% & 58.24\% & 53.83\% \\
        & $|$\MADD{$D$}{D} $-$ \MADD{$D$}{\rBasen{}}$|$  
        & 0.65\% & 0.78\% & 0.41\% & 1.93\% & 0.51\% \\
        & $\Delta$\MADD{$D$}{} $/$ \MADD{$D$}{D} 
        & 0.73\% & 0.89\% & 0.61\% & 3.20\% & 0.93\% \\
        \bottomrule
      \end{tabular}
      \label{tab:bn_noise}
\end{table}


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/BN_ratio_noise.jpg}
\end{center}   
\caption{Curve for noise. Showing the MA percentage difference is nearly positive related to the the BN statistics percentage difference, including mean and std.}
\label{fig:BN_ratio_noise}
\end{figure}


\begin{table}[ht]
      \centering
      \caption{\BN{} statistics results of the distortion effect. The \ltwo{} norm of \MADD{\rBase{}}{D} and \MADD{$D$}{\rBasen{}} to the baseline \BNDD{$R$}{\rBasen{}}, using the corresponding mean and standard deviation values are reported. In both (a) and (b), the absolute \MA{} difference is also shown for comparison. We find that when increasing the distortion level of test dataset (a), the \ltwo{} norm increases as the absolute \MA{} difference increases. However, when increasing the distortion level of the training dataset (b), similar behavior is not shown. In addition, changing the distortion level of the training dataset will result in larger \ltwo{} norm than changing the test dataset.}
      \begin{tabular}{cl|cccccc}
        \toprule
        & & &  \multicolumn{3}{c}{ Dataset ($D$)} \\
        & & D1 & D2 & D3 & D4 & D5\\
        \midrule
        & $\|$\BNDDC{\rBase{}}{D}{mean}$\|_2$ & 40.73 & 45.78 & 71.29 & 97.46 & 110.20 \\
        & $\|$\BNDDC{\rBase{}}{D}{mean} $-$ \BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2$ & 1.04 & 18.12 & 53.76 & 83.17 & 97.09 \\
        & $\Delta$\BNDDC{\rBase{}}{}{mean} $/$ $\|$
        \BNDDC{\rBase{}}{\rBasen{}}{mean}$\|_2$ & 2.55\% & 44.40\% & 131.74\% & 203.81\% & 237.91\% \\
        \cmidrule(r){2-7}
        & $\|$\BNDDC{\rBase{}}{D}{std}$\|_2$ & 91.77 & 90.20 & 87.01 & 73.25 & 61.92 \\
    (a) & $\|$\BNDDC{\rBase{}}{D}{std} $-$ \BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2$ & 0.45 & 5.85 & 15.68 & 26.01 & 35.92 \\
        & $\Delta$\BNDDC{\rBase{}}{}{std} $/$ $\|$ \BNDDC{\rBase{}}{\rBasen{}}{std}$\|_2$ & 0.48\% & 6.35\% & 17.04\% & 28.26\% & 39.03\% \\
        \cmidrule(r){2-7}
        & \MADD{\rBase{}}{D}  & 88.63\% & 74.97\% & 57.67\% & 48.83\% & 49.16\% \\
        & $|$\MADD{\rBase{}}{D} $-$ \MADD{\rBase{}}{\rBasen{}}$|$ & 0.27\% & 13.39\% & 30.69\% & 39.53\% & 39.2\% \\
        & $\Delta$\MADD{\rBase{}}{} $/$ \MADD{\rBase{}}{\rBasen{}} & 0.30\% & 15.15\% & 34.73\% & 44.73\% & 44.36\% \\
        \midrule
        %Element & (B1, R) & (B2, R) & (B3, R) & (B4, R) & (B5, R)\\
        %\midrule
        & $\|$\BNDDC{$D$}{D}{mean}$\|_2$ 
        & 28.42 & 37.90 & 42.30 & 32.86 & 25.60 \\
        & $\|$\BNDDC{$D$}{\rBasen{}}{mean}$\|_2$ 
        & 28.44 & 34.59 & 31.02 & 30.38 & 23.18 \\
        & $\|$\BNDDC{$D$}{D}{mean} $-$ \BNDDC{$D$}{\rBasen{}}{mean}$\|_2$ 
        & 0.68 & 11.31 & 29.21 & 28.22 & 28.22 \\
        & $\Delta$\BNDDC{$D$}{}{mean} $/$ $\|$ \BNDDC{$D$}{D}{mean}$\|_2$  
        & 2.39\% & 29.85\% & 69.06\% & 85.87\% & 110.23\% \\
        \cmidrule(r){2-7}
        & $\|$\BNDDC{$D$}{D}{std}$\|_2$ 
        & 63.15 & 79.72 & 67.69 & 43.47 & 28.83 \\
    (b) & $\|$\BNDDC{$D$}{\rBasen{}}{std}$\|_2$ 
        & 63.31 & 80.88 & 76.00 & 61.05 & 51.97 \\
        & $\|$\BNDDC{$D$}{D}{std} $-$ \BNDDC{$D$}{\rBasen{}}{std}$\|_2$ 
        & 0.31 & 3.94 & 11.40 & 19.51 & 25.42 \\
        & $\Delta$\BNDDC{$D$}{}{std} $/$ $\|$ \BNDDC{$D$}{D}{std}$\|_2$ 
        & 0.49\% & 4.94\% & 16.85\% & 44.87\% & 88.19\% \\
        \cmidrule(r){2-7}
        & \MADD{$D$}{D} 
        & 88.92\% & 89.01\% & 86.36\% & 86.51\% & 85.83\% \\
        & \MADD{$D$}{\rBasen{}} 
        & 88.6\% & 75.56\% & 61.1\% & 54.49\% & 42.97\% \\
        & $|$\MADD{$D$}{D} $-$ \MADD{$D$}{\rBasen{}}$|$  
        & 0.32\% & 13.45\% & 25.26\% & 32.02\% & 42.86\% \\
        & $\Delta$\MADD{$D$}{} $/$ \MADD{$D$}{D} 
        & 0.36\% & 15.11\% & 29.25\% & 37.01\% & 49.93\% \\
        \bottomrule
      \end{tabular}
      \label{tab:bn_distortion}
\end{table}

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/BN_ratio_distortion.jpg}
\end{center}   
\caption{Curve for distortion. Showing the MA percentage difference is nearly positive related to the the BN statistics percentage difference, including mean and std.}
\label{fig:BN_ratio_distortion}
\end{figure}


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/MA_BN_diff_relation.jpg}
\end{center}   
\caption{Data points, showing the relationship between MA percentage difference and BN statistics percentage difference. Overall, the trend of different factor look different (only the noise and distortion factor have similar trend in the left figure). }
\label{fig:BN_ratio_distortion}
\end{figure}


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/MA_BN_diff_relation_circle.png}
\end{center}   
\caption{Data points, showing the relationship between MA percentage difference and BN statistics percentage difference. Red circles are "blur" factor, green circles are "noise" factor, blue circles are "distortion" factor. }
\label{fig:BN_ratio_distortion}
\end{figure}

==> sections/old1/5.2-results.tex <==
\subsection{FID}

In this section we show a metric that is related to the performance loss, so in practice we can use this metric to approximately estimate the performance loss.



\begin{table}[h]
  \caption{Fréchet Inception Distance between R and different datasets with different levels for different factors.}
  \label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|ccccc}
    \toprule
      & Lv1 & Lv2 & Lv3 & Lv4 & Lv5\\
    \midrule
            Blur & 43.64 & 105.08 & 214.56 & 316.87 & 358.54 \\
            Noise & 24.60 & 104.29 & 268.03 & 354.36 & 399.85 \\
            Distortion & 13.33 & 80.94 & 165.65 & 232.34 & 292.31 \\
    \bottomrule
  \end{tabular}
\end{table}


% \begin{table}[h]
%   \caption{Fréchet Inception Distance between different datasets with different blur level.}
%   \label{tab_style_driving_unit}
%   \centering
%   \begin{tabular}{c|cccccc}
%     \toprule
%       & \rBase{} & B1 & B2 & B3 & B4 & B5\\
%     \midrule
%             \rBase{} & 0 & 43.64 & 105.08 & 214.56 & 316.87 & 358.54 \\
%             B1 & 43.64 & 0 & 38.21 & 146.38 & 255.64 & 296.13 \\
%             B2 & 105.08 & 38.21 & 0 & 63.60 & 175.87 & 228.70 \\
%             B3 & 214.56 & 146.38 & 63.60 & 0 & 72.10 & 141.76 \\
%             B4 & 316.87 & 255.64 & 175.87 & 72.10 & 0 & 48.24 \\
%             B5 & 358.54 & 296.13 & 228.70 & 141.76 & 48.24 & 0 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\textwidth]{figures/FID_blur_combine.jpg}
% \end{center}   
% \caption{Fréchet Inception Distance between different datasets with different blur level.}
% \label{fig:BN_ratio_distortion}
% \end{figure}


% \begin{table}[h]
%   \caption{Fréchet Inception Distance between different datasets with different noise level.}
%   \label{tab_style_driving_unit}
%   \centering
%   \begin{tabular}{c|cccccc}
%     \toprule
%       & \rBase{} & N1 & N2 & N3 & N4 & N5\\
%     \midrule
%             \rBase{} & 0 & 24.60 & 104.29 & 268.03 & 354.36 & 399.85 \\
%             N1 & 24.60 & 0 & 53.82 & 217.28 & 316.44 & 372.36 \\
%             N2 & 104.29 & 53.82 & 0 & 92.83 & 207.42 & 284.48 \\
%             N3 & 268.03 & 217.28 & 92.83 & 0 & 68.05 & 169.34 \\
%             N4 & 354.36 & 316.44 & 207.42 & 68.05 & 0 & 45.31 \\
%             N5 & 399.85 & 372.36 & 284.48 & 169.34 & 45.31 & 0 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}[h]
%   \caption{Fréchet Inception Distance between different datasets with different distortion level.}
%   \label{tab_style_driving_unit}
%   \centering
%   \begin{tabular}{c|cccccc}
%     \toprule
%       & \rBase{} & D1 & D2 & D3 & D4 & D5\\
%     \midrule
%             \rBase{} & 0 & 13.33 & 80.94 & 165.65 & 232.34 & 292.31 \\
%             D1 & 13.33 & 0 & 45.71 & 139.30 & 217.14 & 284.24 \\
%             D2 & 80.94 & 45.71 & 0 & 84.91 & 186.42 & 270.23 \\
%             D3 & 165.65 & 139.30 & 84.91 & 0 & 58.24 & 144.07 \\
%             D4 & 232.34 & 217.14 & 186.42 & 58.24 & 0 & 51.28 \\
%             D5 & 292.31 & 284.24 & 270.23 & 144.07 & 51.28 & 0 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table}[h]
  \caption{Fréchet Inception Distance between R and different datasets with different levels for different factors.}
  \label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|ccccc}
    \toprule
      & Darker Lv2 & Darker Lv1 & Lighter Lv1 & Lighter Lv2 \\
    \midrule
            R & 62.71 & 28.40 & 49.79 & 127.52 \\
            G & 95.85 & 44.88 & 97.04 & 165.87 \\
            B & XXX & XXX & XXX & XXX \\
            H & XXX & XXX & XXX & XXX \\
            S & XXX & XXX & XXX & XXX \\
            V & XXX & XXX & XXX & XXX \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/FID_MA.jpg}
\end{center}   
\caption{The relationship between FID and MA percentage difference. }
\label{fig:BN_ratio_distortion}
\end{figure}


% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\textwidth]{figures/MA_BN_diff_relation_circle.jpg}
% \end{center}   
% \caption{Data points, showing the relationship between MA percentage difference and BN statistics percentage difference. The radius of the circle show the BN std difference. "blur" factor is in blue, "noise" factor is in green, "distortion" factor in red. }
% \label{fig:BN_ratio_distortion}
% \end{figure}

==> sections/old1/5.2-results2.tex <==

\begin{table}[h]
  \caption{Fréchet Inception Distance between different datasets with different blur level.}
  \label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
      & \rBase{} & B1 & B2 & B3 & B4 & B5\\
    \midrule
            \rBase{} & 0 & 43.64 & 105.08 & 214.56 & 316.87 & 358.54 \\
            B1 & 43.64 & 0 & 38.21 & 146.38 & 255.64 & 296.13 \\
            B2 & 105.08 & 38.21 & 0 & 63.60 & 175.87 & 228.70 \\
            B3 & 214.56 & 146.38 & 63.60 & 0 & 72.10 & 141.76 \\
            B4 & 316.87 & 255.64 & 175.87 & 72.10 & 0 & 48.24 \\
            B5 & 358.54 & 296.13 & 228.70 & 141.76 & 48.24 & 0 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/FID_blur_combine.jpg}
\end{center}   
\caption{Fréchet Inception Distance between different datasets with different blur level.}
\label{fig:BN_ratio_distortion}
\end{figure}


\begin{table}[h]
  \caption{Fréchet Inception Distance between different datasets with different noise level.}
  \label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
      & \rBase{} & N1 & N2 & N3 & N4 & N5\\
    \midrule
            \rBase{} & 0 & 24.60 & 104.29 & 268.03 & 354.36 & 399.85 \\
            N1 & 24.60 & 0 & 53.82 & 217.28 & 316.44 & 372.36 \\
            N2 & 104.29 & 53.82 & 0 & 92.83 & 207.42 & 284.48 \\
            N3 & 268.03 & 217.28 & 92.83 & 0 & 68.05 & 169.34 \\
            N4 & 354.36 & 316.44 & 207.42 & 68.05 & 0 & 45.31 \\
            N5 & 399.85 & 372.36 & 284.48 & 169.34 & 45.31 & 0 \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[h]
  \caption{Fréchet Inception Distance between different datasets with different distortion level.}
  \label{tab_style_driving_unit}
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
      & \rBase{} & D1 & D2 & D3 & D4 & D5\\
    \midrule
            \rBase{} & 0 & 13.33 & 80.94 & 165.65 & 232.34 & 292.31 \\
            D1 & 13.33 & 0 & 45.71 & 139.30 & 217.14 & 284.24 \\
            D2 & 80.94 & 45.71 & 0 & 84.91 & 186.42 & 270.23 \\
            D3 & 165.65 & 139.30 & 84.91 & 0 & 58.24 & 144.07 \\
            D4 & 232.34 & 217.14 & 186.42 & 58.24 & 0 & 51.28 \\
            D5 & 292.31 & 284.24 & 270.23 & 144.07 & 51.28 & 0 \\
    \bottomrule
  \end{tabular}
\end{table}



\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/FID_MA.jpg}
\end{center}   
\caption{The relationship between FID and MA percentage difference. }
\label{fig:BN_ratio_distortion}
\end{figure}


\begin{figure}[h]
\begin{center}
  \includegraphics[width=\textwidth]{figures/MA_BN_diff_relation_circle.jpg}
\end{center}   
\caption{Data points, showing the relationship between MA percentage difference and BN statistics percentage difference. The radius of the circle show the BN std difference. "blur" factor is in blue, "noise" factor is in green, "distortion" factor in red. }
\label{fig:BN_ratio_distortion}
\end{figure}

==> sections/old1/5.3-results.tex <==

%For example, let $\theta_{noise}$ represent the parameter for noise ($\theta_{noise}$ is a subvector of $\theta_f$), discretize it into $k$ different values in the domain.




% \begin{table}[ht]
%   \caption{For quality and channel factor, we can see some of the test results are improved by combining the original data and modified data (baseline 88.36\%), which means we can use them as data augment method. For the format factor, we can achieve close to the original performance while only use limited information like laplacian map (84.73\%).}
%   \label{tb:style_driving_comb}
%   \centering
%   \begin{tabular}{l|c|ccc}
%     \toprule
%     & Model $M$ & \MARM{} &  &  \\
%     \midrule
%         & \train(\rBase{} + B5) & \textbf{89.67\%} & 89.13\% & \\
% quality  & \train(\rBase{} + N5) & \textbf{90.02\%} & 83.57 \% & \\
%         & \train(\rBase{} + D5) & 87.67\% & 60.20\% & \\
%     \midrule
%         & \train(\rBase{} + channelR) & 88.18\% & 88.33\% & 88.27\%\\
%         & \train(\rBase{} + channelG) & \textbf{90.80\%} & 90.81\% & 90.83\%\\
% channel  & \train(\rBase{} + channelB) & xxx\% & xxx\% & xxx\%\\
%         & \train(\rBase{} + channelH) & 86.66\% & 86.78\% & 87.02\%\\
%         & \train(\rBase{} + channelS) & 86.54\% & 88.24\% & 87.91\%\\
%         & \train(\rBase{} + channelV) & xxx\% & xxx\% & xxx\%\\
% %     \midrule
% %         %& \train(\rBase{} + A) & 75.74\% & 53.34\% & \\
% %         & \train(laplacian) & 35.20\% & 84.73\% \\
% % format  & \train(combmap) & 41.72\% & 85.32\% \\
% %         & \train(\rBase{} + laplacian) & 85.26\% & 82.55\% \\
% %         & \train(\rBase{} + combmap) & 87.44\% & 88.39\% \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% \begin{table}[ht]
%     \caption{From the table we can find our unified discretized adversarial training process can not only help to improve the performance on the original domain $R$, and also help to improve the robustness, i.e., improve the performance on different level noise datasets.}
%   \centering
%   \begin{tabular}{c|cccccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{6}{c}{Test}                   \\
%     \cmidrule(r){2-7}
%     \multicolumn{1}{c}{Train} & \rBase{} & N1 & N2 & N3 & N4 & N5 \\
%     \midrule
%             R (baseline) & 88.36\% & 88.33\% & 86.01\% & 81.42\% & 76.39\% & 73.15\% \\
%             %R+N1+N2+...+N5 (6x time) & 88.89\% & 88.95\% & \textbf{88.98\%} & \textbf{88.83\%} & \textbf{87.47\%} & \textbf{84.67\%} \\
%             % R+Rob(N1\textasciitilde N5) (2x time) & \textbf{89.76\%} & \textbf{89.13\%} & 88.45\% & 87.38\% & 85.62\% & 83.03\% \\
%             R+Rob(N1\textasciitilde N5) & 89.76\% & 89.13\% & 88.45\% & 87.38\% & 85.62\% & 83.03\% \\
%             %R+N5 & 90.03 & 89.85 & 88.24 & 87.61 & 85.53 & 83.57 \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% \begin{table}[ht]
%   \caption{For quality and channel factor, we can see some of the test results are improved by combining the original data and modified data (baseline 88.36\%), which means we can use them as data augment method. For the format factor, we can achieve close to the original performance while only use limited information like laplacian map (84.73\%).}
%   \label{tb:style_driving_comb}
%   \centering
%   \begin{tabular}{l|c|cccccc}
%     \toprule
%   training & factor & original & Lv.1 & Lv.2 & Lv.3 & Lv.4 & Lv.5\\
%     \midrule
%         & blur & 88.36\% & 88.21\% & 88.06\% & 86.07\% & 81.16\% & 73.33\% \\
% R       & noise & 88.36\% & 88.33\% & 86.01\% & 81.42\% & 76.39\% & 73.15\% \\
%         & distortion & 88.36\% & 88.63\% & 74.97\% & 57.67\% & 48.83\% & 49.16\% \\
%     \midrule
%         & blur & 90.32\% & 90.32\% & 90.41\% & 90.29\% & 89.82\% & 85.41\% \\
% R + Rob(B1\textasciitilde B5, N1\textasciitilde N5, D1\textasciitilde D5)  
%         & noise & 90.32\% & 90.56\% & 89.55\% & 89.10\% & 86.66\% & 82.61\% \\
%         & distortion & 90.32\% & 90.08\% & 84.82\% & 80.11\% & 86.42\% & 57.53\% \\
%     \midrule
%         & blur & 1.96\% & 2.11\% & 2.35\% & 4.22\% & 8.66\% & 12.08\% \\
% (Improvement)  
%         & noise & 1.96\% & 2.23\% & 3.54\% & 7.68\% & 10.27\% & 9.46\% \\
%         & distortion & 1.96\% & 1.45\% & 9.85\% & 22.44\% & 37.59\% & 8.37\% \\
%     \midrule
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table}[ht]
  \caption{Improvement for single factor robustness training.}
  \label{tb:style_driving_comb}
  \centering
  \begin{tabular}{l|c|cccccc}
    \toprule
   training & factor & original & Lv.1 & Lv.2 & Lv.3 & Lv.4 & Lv.5\\
    \midrule
Rob(B) & blur & 1.31\% & 1.49\% & 1.31\% & 3.84\% & 7.94\% & 14.21\% \\
Rob(N) & noise & 1.4\% & 0.8\% & 2.44\% & 5.96\% & 9.23\% & 9.88\% \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[ht]
  \caption{
  %Robustness training on quality and channel factors. In this training process, we train the model on all the blur, noise, distortion, G-channel on RGB space (Lv.1 means darker on this channel, and Lv.2 means lighter on this channel, same for the following), S-channel on HSV space, and Y-channel on YUV space, and the results show that the performance can be improved on all levels of all factors.
  Improvement for multi-factor robustness training.}
  \label{tb:style_driving_comb}
  \centering
  \begin{tabular}{l|c|cccccc}
    \toprule
   training & factor & original & Lv.1 & Lv.2 & Lv.3 & Lv.4 & Lv.5\\
    \midrule
%         & blur & 88.36\% & 88.21\% & 88.06\% & 86.07\% & 81.16\% & 73.33\% \\
% R       & noise & 88.36\% & 88.33\% & 86.01\% & 81.42\% & 76.39\% & 73.15\% \\
%         & distortion & 88.36\% & 88.63\% & 74.97\% & 57.67\% & 48.83\% & 49.16\% \\
%         & G-channel(RGB) & 88.36\% & 53.54\% & 51.16\% & - & - & - \\
%         & S-channel(HSV) & 88.36\% & 73.00\% & 61.36\% & - & - & - \\
%         & Y-channel(YUV) & 88.36\% & 46.90\% & 51.25\% & - & - & - \\
%     \midrule
% R+Rob(B)& blur & 89.67\% & 89.70\% & 89.37\% & 89.91\% & 89.10\% & 87.54\% \\
% R+Rob(N)& noise & 89.76\% & 89.13\% & 88.45\% & 87.38\% & 85.62\% & 83.03\% \\
%     \midrule
%         & blur & 89.76\% & 89.76\% & 90.08\% & 90.29\% & 89.37\% & 87.67\% \\
%         & noise & 89.76\% & 90.00\% & 89.52\% & 88.72\% & 87.17\% & 84.16\% \\
% R + Rob(B, N, D, G, S, Y)           
%         & distortion & 89.76\% & 89.43\% & 82.11\% & 77.94\% & 84.58\% & 60.62\% \\
%         & G-channel(RGB) & 89.76\% & 88.72\% & 90.38\% & - & - & - \\
%         & S-channel(HSV) & 89.76\% & 83.30\% & 88.42\% & - & - & - \\
%         & Y-channel(YUV) & 89.76\% & 79.52\% & 88.86\% & - & - & - \\
%     \midrule
        & blur & 1.4\% & 1.55\% & 2.02\% & 4.22\% & 8.21\% & 14.34\% \\
        & noise & 1.4\% & 1.67\% & 3.51\% & 7.3\% & 10.78\% & 11.01\% \\
Rob(B, N, D, G, S, Y) & distortion & 1.4\% & 0.8\% & 7.14\% & 20.27\% & 35.75\% & 11.46\% \\
        & G-channel(RGB) & 1.4\% & 35.18\% & 39.22\% & - & - & - \\
        & S-channel(HSV) & 1.4\% & 10.3\% & 27.06\% & - & - & - \\
        & Y-channel(YUV) & 1.4\% & 32.62\% & 37.61\% & - & - & - \\
    \midrule
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[ht]
  \caption{Comparison between different methods. Avg represents the average improvement on all levels of all factors.}
  \label{tb:style_driving_comb}
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
   method & Avg & Min & Max & Time\\
    \midrule
data augmentation & xxx\% & xxx\% & xxx\% & xxx\\
Adversarial training & xxx\% & xxx\% & xxx\% & xxx\\
Online Hard Example Mining & xxx\% & xxx\% & xxx\% & xxx\\
Maxup & xxx\% & xxx\% & xxx\% & xxx\\
ours & xxx\% & xxx\% & xxx\% & xxx\\
    \bottomrule
  \end{tabular}
\end{table}


==> sections/old1/learning-results_backup.tex <==
\subsection{Experiments and Results}
\label{results}
All experiments are conducted using Intel(R) Xeon(TM) W-2123 CPU, Nvidia GTX 1080 GPU, and 32G RAM. We use the Adam optimizer~\citep{kingma2014adam} with learning rate 0.0001 and batch size 128 for training. The maximum number of epochs is 1000. 
Images in the base dataset are sampled from videos at 30 frames per second (FPS). For efficiency, we adopt a similar approach as in \citet{bojarski2016end} by further downsampling the dataset to 5 FPS to reduce similarities between adjacent frames. The resulting dataset contains approximately 10,000 images. We randomly split the dataset with about 20:1:2 as training/validation/test data.

We compare our method with three methods: a baseline method~\citep{bojarski2016end}, an adversarial training method~\citep{shu2020preparing}, and a na\"{i}ve data augmentation method. For the na\"{i}ve data augmentation method, we simply merge all perturbed datasets together to train the model. We test the performance of all methods in four scenarios with increasing complexity:

% For the adversarial training method, we use a recent method by Shu et al.~\citep{shu2020preparing}, where feature space adversarial training is used to achieve generalization to variant image perturbations. 


% \begin{itemize}
%     \item Scenario 1: Base dataset. Test on the base dataset.
%     \item Scenario 2: Single perturbation. Test on the datasets with different level of different perturbations, but each dataset only has one level of one perturbation (within blur, noise, distortion, R, G, ,B, H, S, V).
%     \item Scenario 3: Combined perturbation. Test on the datasets with combinations of different level of different perturbations, and each dataset have different level of all the perturbation (within blur, noise, distortion, R, G, ,B, H, S, V).
%     \item Scenario 4: Unseen perturbation. Test on the datasets with unseen perturbations in different level. Specifically, we use "motion blur", "zoom blur", "pixelate", "jpeg compression", "snow", "frost", "fog" from ImageNet-C~\citep{hendrycks2019benchmarking}.
% \end{itemize}

% For Scenario 1, we use the base dataset[] directly. For Scenario 2, we use 5 levels for blur (Gaussian blur), noise, distortion, and 10 levels for R, G, B, H, S, V, as we described in Sec.\ref{sec:ssensitivity_analysis}. For Scenario 3, we randomly sample different levels for different kinds of perturbations in Scenario 2 and apply them onto one dataset, which forms one combination dataset. We sample 6 combination datasets in this test scenario. See examples in the second row Fig.\ref{fig:salience_map}. For For Scenario 4, we use "motion blur", "zoom blur", "pixelate", "jpeg compression", "snow", "frost", "fog" from ImageNet-C~\citep{hendrycks2019benchmarking}, since "motion blur" and "zoom blur" are possible to happen during driving, "pixelate" and "jpeg compression" are possible to happen during image processing, and "snow", "frost", "fog" are weather conditions, all of them are related to our application but is different from the 9 basic factors that we are chosen. Notice for the blur factor, what we use is Gaussian blur, which is different with motion blur and zoom blur. See examples in Fig.\ref{fig:unseen_factors}.

\begin{itemize}
    \item Scenario 1: \emph{Clean data}. Test on the base clean dataset only.
    \item Scenario 2: \emph{Single Perturbation}. Test on datasets of each factor at its discretized levels. Specifically, we use five levels for blur, noise, distortion, and ten levels for R, G, B, H, S, V. Hence, we have 75 datasets in total for testing in this scenario. 
    \item Scenario 3: \emph{Combined Perturbation}. Test on datasets with combinations of all factors at all levels. To be specific, we sample varying levels from each factor, and combine the resulting datasets of all factors into one \emph{combined} dataset. In total, we have six \emph{combined} datasets for testing in this scenario. See examples in the second row of Figure~\ref{fig:salience_map}, and parameters for each dataset in the appendix section~\ref{app:perturbed-datasets}.
    \item Scenario 4: \emph{Unseen Perturbation}. Test on datasets under previously unseen factors at different levels. The unseen factors are ``motion blur'', ``zoom blur'', ``pixelate'', ``jpeg compression'', ``snow'', ``frost'', ``fog'' from ImageNet-C~\citep{hendrycks2019benchmarking}. We choose these factors because, specifically, ``Motion blur'' and ``zoom blur'' can happen during driving; ``pixelate'' and ``jpeg compression'' are possible during image processing; and ``snow'', ``frost'', ``fog'' are natural weather conditions that can affect driving experiences. In addition, all these factors can be possibly ``simulated'' using the nine image factors analyzed in this work. 
    % (although for blurr, we use Gaussian blur, which is different with motion blur and zoom blur. 
    See examples in Figure~\ref{fig:unseen_factors}.
\end{itemize}

% Scenario 1: \emph{Base Dataset}. Test on the base dataset only.

% Scenario 2: \emph{Single Perturbation}. Test on the datasets with different levels of dperturbations and each dataset only has one level of perturbation. Specifically, we use 5 levels for blur (Gaussian blur), noise, distortion, and 10 levels for R, G, B, H, S, V, as we described in Sec.~\ref{sec:ssensitivity_analysis}.

% Scenario 3: \emph{Combined Perturbation}. Test on the datasets with combinations of different levels of varying perturbations, and each dataset have different levels of all  perturbations (within blur, noise, distortion, R, G, ,B, H, S, V). we randomly sample different levels to create different kinds of perturbations from Scenario 2 and combine them into one dataset. We sample 6 combination datasets in this test scenario. See examples in the second row of Fig.~\ref{fig:salience_map}. 

% Scenario 4: \emph{Unseen Perturbation}. Test on the datasets with unseen perturbations in different levels. Specifically, we use "motion blur", "zoom blur", "pixelate", "jpeg compression", "snow", "frost", "fog" from ImageNet-C~\citep{hendrycks2019benchmarking}, since "motion blur" and "zoom blur" can happen during driving, "pixelate" and "jpeg compression" are possible during image processing, and "snow", "frost", "fog" are due too weather conditions.  All of them are related to our application but can be possibly simulated from some combination of 9 image quality factors chosen. Notice for the blur factor, what we use is Gaussian blur, which is different with motion blur and zoom blur. See examples in Fig.~\ref{fig:unseen_factors}.

\begin{figure}[h]
\begin{center}
  \includegraphics[width=\linewidth]{figures/unseen_factors.jpg}
\end{center}   
% \vspace*{-1em}
\caption{Unseen perturbation examples in our experiments. We use ``snow'', ``frost'', ``fog'' (left to right; first row), and ``motion blur'', ``zoom blur'', ``pixelate'', ``jpeg compression'' (left to right; second row) from the corruptions in ImageNet-C~\citep{hendrycks2019benchmarking}. 
}
\label{fig:unseen_factors}
\end{figure}


We use the maximum MA improvement (denoted as MMAI), the average MA improvement (denoted as AMAI) and mean Corruption Errors (mCE)~\citep{hendrycks2019benchmarking} as the evaluation metrics. 
From Table~\ref{tb:overall_results}, we observe that our method outperforms other methods under all metrics in all scenarios. Specifically, our algorithm improves the performance of ``learning to steer'' up to 48\% in MMAI, while reducing mCE down by 50\% over the baseline. We have compared our approach with other related techniques, namely data augmentation and adversarial training. The results show that our method achieves consistent better performance. Our method also improves the task performance using the \emph{combined} datasets (Scenario 3) up to 33\%. Lastly, when tested on unseen factors (Scenario 4), our algorithm maintains the best performance by 29\% in MMAI, while reducing mCE error to 76\%.

% \begin{table}[ht]
%   \caption{Comparison between different method under different test scenarios. $\Delta$mMA stands for the average MA improvement, compare with the baseline method. mCE stands for mean corruption errors\citep{hendrycks2019benchmarking}. We can see our method outperform others with both metrics in all scenarios. (\%)}
%   \label{tb:style_driving_comb}
%   \centering
%   \begin{tabular}{c|cc|cc|cc}
%     \toprule
%      Scenario & \multicolumn{2}{c}{Single Perturbation} & \multicolumn{2}{c}{Combined Perturbation} & \multicolumn{2}{c}{Unseen Perturbation} \\
%     \midrule
%   method& $\Delta$mMA & mCE & $\Delta$mMA & mCE & $\Delta$mMA & mCE\\
%     \midrule
% Adversarial training[] & 10.61 & 74.42 & 6.99 & 86.82 & 8.17 & 89.91\\
% Our data + Basic training & 19.97 & 51.34 & 11.97 & 75.84 & 7.92 & 81.51 \\
% % Online Hard Example Mining & xxx\% & xxx\% & xxx\% & xxx\\
% % Maxup & xxx\% & xxx\% & xxx\% & xxx\\
% ours & \textbf{20.74} & \textbf{49.47} & \textbf{17.74} & \textbf{63.81} & \textbf{9.06} & \textbf{76.20} \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table*}[ht]
  \centering
  \scalebox{.8}{
  \begin{tabular}{c|c|ccc|ccc|ccc}
    \toprule
    & \multicolumn{10}{c}{Scenarios} \\
        \midrule
      & \multicolumn{1}{c}{Clean} & \multicolumn{3}{c}{Single Perturbation} & \multicolumn{3}{c}{Combined Perturbation} & \multicolumn{3}{c}{Unseen Perturbation} \\
    \midrule
   Method& AMAI$\uparrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$\\
    \midrule
    
Data Augmentation & -0.44 & 46.88 & 19.97 & 51.34 & \textbf{36.1}  & 11.97 & 75.84 & 27.5  & 7.92 & 81.51 \\
Adversarial Training & -0.65 & 30.06 & 10.61 & 74.42 & 17.89  & 6.99 & 86.82 & 16.9  & 8.17 & 89.91\\
Maxup & -7.79 & 38.30 & 12.83 & 66.56 & 26.94 & 16.01 & 72.60 & 23.43 & 5.54 & 81.75\\
AugMix & -5.23 & 40.27 & 15.01 & 67.49 & 26.81 & 15.45 & 68.38 & 28.70 & 8.85 & 87.79\\
Ours & \textbf{0.93} & \textbf{48.57} & \textbf{20.74} & \textbf{49.47} & 33.24  & \textbf{17.74} & \textbf{63.81} & \textbf{29.32}  & \textbf{9.06} & \textbf{76.20} \\
    \bottomrule
  \end{tabular}}
 \caption{Performance improvement comparison of different methods in four scenarios against the baseline performance on Chen's dataset, using the maximum MA improvement in percentage (denoted as MMAI), the average MA improvement in percentage (denoted as AMAI), and mean corruption errors in percentage (mCE). For adversarial training, we use the state-of-the-art method described in~\citep{shu2020preparing}. For data augmentation, we simply combine all perturbed datasets into training. As a result, our method outperforms the other methods (highest MA improvements and lowest mCEs) in nearly all scenarios.}
  \label{tb:overall_results}
\end{table*}





% \begin{figure}\CenterFloatBoxes
%     \begin{floatrow}
%     \ffigbox[\FBwidth] {
%     \caption{figure caption goes here}\label{fig: figure-label}}
%     \includegraphics[width=10cm, height=4cm]{figures/boxplot.png}
%     \killfloatstyle\ttabbox[\Xhsize]
%     {\caption{table caption goes  here}\label{tab: table-label}}
%     \begin{tabular}{c|ccc}
%     \toprule
%         method & single & combined & unseen \\
%         \midrule
%         Adv & 74.42 & 86.82 & 89.91 \\
%         Aug & 51.34 & 75.84 & 81.51 \\
%         Ours & 49.47 & 63.81 & 76.20 \\
%     \bottomrule
%     \end{tabular}
%     \end{floatrow}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=10cm, height=4cm]{figures/boxplot.png}
%     \caption{Comparison between different methods under different test scenarios, based on MA improvements. For each test dataset, the corresponding Maximum MA Improvement, the Median MA improvement, and Minimum MA Improvements are visualized as boxplots.  We observe that the distribution of MA improvement on our method is generally higher with less variance. }
%     \label{fig:boxplot_ma_improvement}
%     \vspace*{-1em}
% \end{figure}

% \begin{table}[H]
%    \centering
%    \caption{mCE values for each pairwise test scenario (single, combined, unseen) and method (adversarial training, data augmentation, our method). (\%)}
%    \label{tab:mce_table_simple}
%    \begin{tabular}{c|ccc}
%    \toprule
%        method & single & combined & unseen \\
%        \midrule
%        Adv & 74.42 & 86.82 & 89.91 \\
%        Aug & 51.34 & 75.84 & 81.51 \\
%        Ours & 49.47 & 63.81 & 76.20 \\
%    \bottomrule
%    \end{tabular}
% \end{table}

We also illustrate the detailed MA improvements in Fig.~\ref{fig:MA_channel_unseen_improvement}, which shows that our method can achieve improvements in some extreme cases of the channel-factor levels and some of the unseen image effects. However, our method fails to improve on ``motion blur'', which we plan to study in future. More detailed data, results, and analysis can be found in Appendix~\ref{Apd:experiment_data}.

\begin{figure*}[h]
\begin{center}
  \includegraphics[width=0.9\linewidth]{figures/MA_channel_unseen_improvement.jpg}
\end{center}   
% \vspace*{-1em}
\caption{MA improvement with our method compared to the baseline. Our method achieve great improvement on extreme cases for channel-level factors and unseen weather conditions.}
\label{fig:MA_channel_unseen_improvement}
%\vspace*{-1em}
\end{figure*}

By visualizing the salience map on several combined samples in Fig.~\ref{fig:salience_map}, we show that our method can assist the network to focus on more important areas (e.g., the road in front), instead of focusing on random areas on perturbed images.

\begin{figure*}[h]
\begin{center}
  \includegraphics[width=0.9\linewidth]{figures/Salience_map.jpg}
\end{center}   
% \vspace*{-1em}
\caption{Saliency map samples with baseline method and our method, where the model tests on the different combinations of perturbations. Different columns show different combinations of perturbations. The first row shows the original image, the second row shows the perturbed image with the chosen effects, the third row is the saliency map of baseline model, and the fourth row is the saliency map of our method. It can be seen that, with our method, the network can better focus on the important areas (e.g., the road in front) instead of random areas on the perturbed images, as with the baseline model. 
% Also, the MA improvements on these datasets are [36.82\%, 12.2\%, 29.05\%, 16.16\%, 35.42\%, 34.7\%] (from left to right in order), which shows our method can also handle combination effects even only use single effect datasets during training.
}
\label{fig:salience_map}
% \vspace*{-1em}
\end{figure*}


\subsection{Wider Comparison}
To show our method can be generalized well in other cases, we show the experiment results on two new datasets (Honda~\citep{ramanishka2018toward} and Audi~\citep{geyer2020a2d2}, see dataset setup in Appendix~\ref{Apd:dataset_setup}), one new method (Augmix~\citep{hendrycks2019augmix}), and one new backbone network (comma.ai~\citep{santana2016learning}) in Table.~\ref{tb:overall_results_honda} and Table.~\ref{tb:overall_results_audi}. As shown in the tables, our method achieves the best performance on most cases. Specifically, our method outperforms on clean and single perturbation data consistently (at least 2.5\% better), and does better in most cases of unseen perturbation data. In combined perturbation data, our method performs better when using NVidia backbone network, while AugMix performs better when using comma.ai backbone network.


\begin{table*}[ht]
  \centering
  \scalebox{.8}{ %\color{blue}
  \begin{tabular}{c|c|ccc|ccc|ccc}
    \toprule
    & \multicolumn{10}{c}{Scenarios} \\
        \midrule
      & \multicolumn{1}{c}{Clean} & \multicolumn{3}{c}{Single Perturbation} & \multicolumn{3}{c}{Combined Perturbation} & \multicolumn{3}{c}{Unseen Perturbation} \\
    \midrule
   Method& AMAI$\uparrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$\\
    \midrule
    
AugMix+Nvidia & -0.12 & 40.64 & 10.94 & 76.48 & 25.97 & 16.79 & 64.41 & \textbf{22.23} & 5.99 & 84.95\\
Ours+Nvidia & \textbf{2.48} & \textbf{43.51} & \textbf{13.51} & \textbf{67.78} & \textbf{28.13} & \textbf{17.98} & \textbf{61.12} & 16.93 & \textbf{6.70} & \textbf{80.92}\\
    \midrule
AugMix+Comma.ai & -5.25 & 55.59 & 9.56 & 86.31 & 31.32 & \textbf{0.77} & \textbf{106.1} & 37.91 & 7.97 & 89.99\\
Ours+Comma.ai & \textbf{0.36} & \textbf{62.07} & \textbf{15.68} & \textbf{70.84} & \textbf{38.01} & 0.74 & 108.32 & \textbf{42.54} & \textbf{12.15} & \textbf{77.08}\\
    \midrule
AugMix+ResNet152 & -4.23 & 20.84 & 1.45 & 96.24 & 12.21 & 6.71 & 80.19 & 15.40 & 2.87 & 97.62\\
Ours+ResNet152 & -0.96 & 24.29 & 5.19 & 79.76 & 16.05 & 8.02 & 75.16 & 16.58 & 5.33 & 85.68\\
%     \midrule
% AugMix+LSTM & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx\\
% Ours+LSTM & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx\\
    \bottomrule
  \end{tabular}}
 \caption{Performance improvement comparison of different backbone network in four scenarios against the baseline performance on Honda dataset. Our method outperforms AugMix in most cases. Notice the methods with ResNet152 do not improve as much as the first two networks because the baseline with ResNet152 already has a relatively high performance.
}
  \label{tb:overall_results_honda}
\end{table*}

% \begin{table*}[ht]
%   \centering
%   \scalebox{.8} { %\color{blue}
%   \begin{tabular}{c|c|ccc|ccc|ccc}
%     \toprule
%     & \multicolumn{10}{c}{Scenarios} \\
%         \midrule
%       & \multicolumn{1}{c}{Clean} & \multicolumn{3}{c}{Single Perturbation} & \multicolumn{3}{c}{Combined Perturbation} & \multicolumn{3}{c}{Unseen Perturbation} \\
%     \midrule
%   Method& AMAI$\uparrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$\\
%     \midrule
    
% AugMix+N & -8.24 & 81.89 & 32.22 & 55.27 & 75.49 & 50.23 & 41.98 & 73.06 & 27.39 & 77.51\\
% Ours+N & \textbf{4.13} & \textbf{94.95} & \textbf{45.78} & \textbf{18.79} & \textbf{80.42} & \textbf{59.31} & \textbf{29.33} & \textbf{75.16} & \textbf{31.91} & \textbf{42.89}\\
%     \midrule
% AugMix+C & -18.7 & 57.23 & 12.71 & 89.74 & 36.88 & \textbf{28.17} & \textbf{68.78} & 37.68 & 4.15 & 119.64\\
% Ours+C & \textbf{-1.33} & \textbf{77.99} & \textbf{30.87} & \textbf{50.81} & \textbf{47.87} & 23.18 & 73.14 & \textbf{42.98} & \textbf{14.15} & \textbf{80.42}\\
%     \bottomrule
%   \end{tabular}}
%  \caption{Comparison on Audi dataset. In "Method" column, "N" means Nvidia backbone network, "C" means comma.ai backbone network. Our method outperforms AugMix in most cases.}
%   \label{tb:overall_results_audi}
% \end{table*}


\begin{table*}[ht]
  \centering
  \scalebox{.8} { %\color{blue}
  \begin{tabular}{c|c|ccc|ccc|ccc}
    \toprule
    & \multicolumn{10}{c}{Scenarios} \\
        \midrule
      & \multicolumn{1}{c}{Clean} & \multicolumn{3}{c}{Single Perturbation} & \multicolumn{3}{c}{Combined Perturbation} & \multicolumn{3}{c}{Unseen Perturbation} \\
    \midrule
  Method& AMAI$\uparrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$ & MMAI$\uparrow$ & AMAI$\uparrow$ & mCE$\downarrow$\\
    \midrule
    
AugMix on Chen's & -5.23 & 40.27 & 15.01 & 67.49 & 26.81 & 15.45 & 68.38 & 28.70 & 8.85 & 87.79\\
Ours on Chen's & \textbf{0.93} & \textbf{48.57} & \textbf{20.74} & \textbf{49.47} & \textbf{33.24}  & \textbf{17.74} & \textbf{63.81} & \textbf{29.32}  & \textbf{9.06} & \textbf{76.20}\\
    \midrule
AugMix on Honda & -0.12 & 40.64 & 10.94 & 76.48 & 25.97 & 16.79 & 64.41 & \textbf{22.23} & 5.99 & 84.95\\
Ours on Honda & \textbf{2.48} & \textbf{43.51} & \textbf{13.51} & \textbf{67.78} & \textbf{28.13} & \textbf{17.98} & \textbf{61.12} & 16.93 & \textbf{6.70} & \textbf{80.92}\\
    \midrule
AugMix on Audi & -8.24 & 81.89 & 32.22 & 55.27 & 75.49 & 50.23 & 41.98 & 73.06 & 27.39 & 77.51\\
Ours on Audi & \textbf{4.13} & \textbf{94.95} & \textbf{45.78} & \textbf{18.79} & \textbf{80.42} & \textbf{59.31} & \textbf{29.33} & \textbf{75.16} & \textbf{31.91} & \textbf{42.89}\\
    
    \bottomrule
  \end{tabular}}
 \caption{Performance comparison on different datasets in four scenarios against the baseline performance.}
  \label{tb:overall_results_audi}
\end{table*}

\subsection{Generalization}
In this work, we introduce an efficient and effective computational framework that incorporates sensitivity analysis and a systematic mechanism to improve the performance of a learning algorithm for autonomous driving on both the original
dataset and the simulated adversarial scenarios due to multiple perturbations defined on an influential set of important image attributes.
This approach can be easily extended and applied beyond the set of factors and the learning algorithm analyzed in this paper.  This method can generalize to analyzing any arbitrarily high number of image/input factors, other learning algorithms, and multimodal sensor data. Furthermore, other autonomous systems where the perception-to-control functionality plays a key role can possibly benefit from such a technique as well.
